Securing Smart Home Edge Devices against Compromised Cloud Servers

Smart home IoT systems often rely on cloud-based servers for communication between components. Although there exists a body of work on IoT security, most of it focuses on securing clients (i.e., IoT devices). However, cloud servers can also be compromised. Existing approaches do not typically protect smart home systems against compromised cloud servers. This paper presents FIDELIUS: a runtime system for secure cloud-based storage and communication even in the presence of compromised servers. FIDELIUS's design is tailored for smart home systems that have intermittent Internet access. In particular, it supports local control of smart home devices in the event that communication with the cloud is lost, and provides a consistency model using transactions to mitigate inconsistencies that can arise due to network partitions. We have implemented FIDELIUS, developed a smart home benchmark that uses FIDELIUS, and measured FIDELIUS's performance and power consumption. Our experiments show that compared to the commercial Particle.io framework, FIDELIUS reduces more than 50% of the data communication time and increases battery life by 2X. Compared to PyORAM, an alternative (ORAM-based) oblivious storage implementation, FIDELIUS has 4-7X faster access times with 25-43X less data transferred.

==> Securing Smart Home Edge Devices against Compromised Cloud Servers/abstract.tex <==
%Smart home IoT systems often rely on cloud-based servers for communication
%between components.  Although there exists a body of work on IoT security, 
%most of it focuses on securing clients (\ie IoT devices) and not on securing
%against compromised cloud servers.
This paper presents \TOOL---a runtime system for secure cloud-based
storage and communication even in the presence of compromised
servers. \TOOL's design is tailored for smart home systems that
have \emph{intermittent Internet access}. In particular, it supports
local control of smart home devices in the event that communication
with the cloud is lost, and provides a consistency model using
transactions to mitigate inconsistencies that can arise due to network
partitions. We have implemented \TOOL, developed a smart home
benchmark that uses \TOOL, and measured \TOOL's performance and power
consumption.  Our experiments show that compared to the commercial Particle.io framework, \TOOL reduces more than \textbf{50\%} of the data communication time and increases battery life by \textbf{2$\times$}.
Compared to PyORAM, an alternative (ORAM-based) oblivious storage implementation, \TOOL
has \textbf{4-7$\times$}
faster access times with \textbf{25-43$\times$} less data transferred. 


==> Securing Smart Home Edge Devices against Compromised Cloud Servers/attack.tex <==
\mysection{Threat Model}\label{sec:threat}

%\todo{NEED TO RE-POSITION THE WORK: BASICALLY FIDELIUS IS ONLY GOOD IF THE DEVICES DON'T NEED A LOT OF SERVER PROCESSING.}
\TOOL focuses on preventing attackers from using compromised servers to mount large scale attacks on smart home devices.
The problem of
client security for smart home devices is thus outside of the scope of this
paper.\footnote{ \TOOL can be easily used together with any existing client-side security enforcement technique to provide a \mycomment{complete} comprehensive
solution to the problem of smart-home IoT security.}
We assume that the adversary has leveraged other vulnerabilities to
obtain complete control over the cloud server that is used by the
devices to communicate.  We assume that the adversary has knowledge
of \TOOL but does not know the secret key to which only the clients have access.

\TOOL provides the following guarantees, which are formalized in the technical report~\cite{technicalreport}: %Appendices~\ref{sec:security} and \ref{sec:proof}:
\squishcount
\item \TOOL provides oblivious privacy.  
%In the absence of message queue resizes, 
\TOOL does not leak any information from data access
patterns.  However, \TOOL may leak information from 
timing.

\item \TOOL guarantees the integrity of the message passing
layer.  It ensures that any violation of integrity is detected by some
client and that even in the case of a detected integrity violation,
the consequences for a client is limited to the same set of
behaviors that are allowed by the non-determinism from the network, \ie
could have arisen with a honest server receiving messages from clients in a different order.
\countend

A malicious server can implement a denial-of-service (DoS)
attack by not forwarding messages.  A malicious server can also
partition clients into disjoint groups that it does not permit to
communicate.  This attack is impossible for a client to distinguish
from a network failure that prevents the server from
communicating with a subset of clients, and thus \TOOL provides
fork consistency~\cite{sundr} by default.  
%We expect that fork consistency suffices for nearly all smart home systems, but the \TOOL approach does support stronger consistency guarantees (at a cost to availability) if needed.  
\mycomment{
Section~\ref{sec:consistency} discusses how \TOOL can
provide strong consistency guarantees than fork consistency.}

%We assume that compromising the server does not allow the attacker to
%rewrite the device firmware with malicious code.  This is reasonable as many real-world IoT devices check firmware update
%signatures using public keys.  
%In principle, it is possible to secure the private 
%firmware signing keys by keeping them on a non-network %connected machine.
%\todo{I think this last sentence is problematic -- if we keep the keys on an isolated machine, how can the devices access them? BD: The devices use the public keys to check signatures...do we need to say more here?}


==> Securing Smart Home Edge Devices against Compromised Cloud Servers/conclusion.tex <==
\mysection{Conclusion}\label{sec:conclusion}

We presented \TOOL, a new secure key-value store, that is
designed to meet the requirements of smart home systems.
We prove that \TOOL is secure, even
in the presence of a malicious cloud server.  
Our experiments show that \TOOL has
good performance, low power consumption, is resilient to attacks, and efficiently runs on
smart home class hardware.  

\mysection{Discussion}\label{sec:discussion}

\myparagraph{Feedback}
%This paper primarily focuses on securing clients against
%malicious cloud server. In particular, 
\TOOL is a
privacy-preserving infrastructure with a specific context
(\ie key-value store).
We are seeking feedback about the viability
of \TOOL in the real-world setting with respect to 
the current trends for cloud architecture.
We are also looking into future directions to extend
\TOOL for more complex applications beyond key-value
store model (\eg cameras and video streaming devices).

\myparagraph{Controversial Points}
First, \TOOL distributes key among devices. However, this could
be a bad choice because the entire system will be compromised
if a client gets compromised.
Second, \TOOL tries to leverage encryption in the communication
between IoT devices---this might be too heavy for IoT devices
that typically have limited resources (\eg processing power
and memory). While a lot of devices have implemented
their communication protocols on top of secure channels, \eg
TLS, there are still devices that communicate in clear text
for simplicity.
Third, \TOOL protects the privacy of clients by concealing 
the data from the cloud server. However, the current trend is
that cloud servers typically access clients' data for analytics purposes.

\myparagraph{Likely Discussion}
We hope that this paper could generate discussions
with the following questions (with respect to the
controversial points and the feedback we look for):
\textbf{(1)} How viable is \TOOL to provide 
privacy and security for IoT devices with respect to current trends and practices? What could be the better scheme to distribute keys
if we use encryption (with the assumption that the cloud server could be malicious)? Could we really trust the clients?
%While some existing devices have been using TLS, could
%there be a more lightweight scheme for low-power devices?
\textbf{(2)} How could we develop \TOOL better in
the direction that follows the current trend for cloud
analytics? \TOOL may not
be suitable for all IoT applications. However, it
can be effective for certain scenarios, in which the user may not want
the server to comprehend the data, 
\eg when a company uses a public cloud service to run its applications, it needs to protect its users' sensitive information. 
We realize that when using \TOOL, 
data analytics can still be performed
using another machine (as a \TOOL client).

\myparagraph{Open Issues}
\TOOL provides security through encryption and
packets with the same-length. However, there is 
still privacy leak through timing channels. 
Although, an obvious solution is 
traffic injection~\cite{cai2014cs,cai2014systematic},
this could consume a lot of bandwidth: inefficient communication.
Thus, we wonder if there could be a more efficient
solution to secure the timing channels for IoT
devices.

\myparagraph{Circumstances for Failure}
%The scalability limit of \TOOL could be a condition
%for failure. 
IoT devices typically have limited processing
power and storage, especially for devices that are
most likely to use the key-value store model.
Thus, if there are too many devices that participate
as a \TOOL client, the message chain can be too
long to fit into the device's local storage. As a result, the entire \TOOL system could fail.

==> Securing Smart Home Edge Devices against Compromised Cloud Servers/eval.tex <==
\mysection{Evaluation}\label{sec:eval}

We developed both C++ and Java implementations of the \TOOL client and
a C++ implementation of the \TOOL 
server.\footnote{
Most existing smart home systems are closed source
and it is not clear what guarantees are provided when there are conflicts.
Thus, we cannot implement our approach to securing smart home devices against malicious cloud servers directly on these devices. 
Instead, we implemented a complete system (with an API library) that uses transactions to support local communication with clear consistency properties.
}
The server for all experiments was a 3.5GHz Intel Xeon E3-1246 v3 with
32GB of RAM.  We have evaluated \TOOL by (1) developing a test bed
system, (2) comparing with the commercial Particle
cloud in terms of energy usage and privacy, and (3) comparing with a Path ORAM implementation~\cite{stefanov-ccs13b}.

%\mysubsection{Test Bed Smart Home System}\label{sec:testbed}

\myparagraph{Test Bed}
Our test bed system simulates a medium scale smart home deployment
with 16 devices.  We have two classes of smart home devices in our
test bed: (1) 15 low-power nodes that use hardware similar to
smart home devices that run on batteries for many months (8 Particle
Photons with temperature and humidity sensors, 4 Particle Photons with
magnetic door sensors, 3 Particle Photons with IR-based motion
sensors) and (2) one mid-range node that uses hardware that is more
typical of smart home devices that run on wall power 
(a Raspberry Pi 1 that controls 2 LiFX smart light bulbs).\footnote{
The Particle Photon is a low-end 
IoT hardware development kit with a 120 MHz ARM Cortex M3
processor, 1MB of flash, and 128KB of RAM that supports 802.11b/g/n
WiFi.}
These specifications are similar to the hardware that appear in commercial devices.  
\mycomment{
For comparison, the Nest Protect battery powered smoke detector
uses a 100 MHz Cortex M4 processor as a primary processor (with 2
other ARM Cortex processors) and thus the Particle Photon is roughly
equivalent to processors in the Nest Protect.
The Raspberry Pi 1 has a 700MHz single core ARM11 processor.  For comparison,
the Nest thermostat contains a 1GHz single core Cortex A8 which is
$\sim2.5\times$ faster than the Raspberry Pi.  Note that we had to use
development kits to run \TOOL since off-the shelf systems are closed source and not modifiable.
}

%\mysubsubsection{CPU Load for Raspberry Pi}
%\myparagraph{CPU Load}
We quantified the CPU overhead of \TOOL for typical smart home device activity (controlling LiFX light bulbs) on a smart home class CPU (a Raspberry Pi 1) to verify that \TOOL incurs acceptable overheads. 
%Our workload used an Android app to issue a command
%to a light bulb every second in a round-robin fashion.  We ran this
%experiment for 1 minute.  
For this experiment, the LiFX arbitrator had
a 2.3\% CPU utilization and the Android app had below 1\% CPU utilization.  
%We did not perform a similar
%measurement on the Particle Photons as they do not have OS support for
%measuring CPU utilization.
%We also validated that local control worked by disconnecting the
%router from the Internet and verifying that the app could still
%control the light bulbs.

%\mysubsubsection{Attacks}
%\mysubparagraph{Attacks}
To validate that \TOOL detects attacks,
we used a malicious server that implements three
different attacks. In the first attack, the server assigns the sequence
number to multiple messages. In the second attack, the server inserts
a rejected message into the queue. In the third attack, the server
swaps message sequence numbers of accepted messages.  \textit{The clients detected all attacks.}

%\mysubsubsection{Energy Measurements \& Comparison to Particle Cloud}\label{sec:energy}
\mycomment{
\begin{table}[th]
  \vspace{-1em}
  \centering
  \begin{center}
  { \footnotesize
  \begin{tabular}{| l | r | r | r | r | r | r |}
    \hline
        Sensor & \multicolumn{3}{| c |}{Particle cloud} & \multicolumn{3}{| c |}{Fidelius cloud}\\
    \cline{2-7}
        Type& Uptime & Energy & Life-  & Uptime & Energy &Life-\\
        & (\textit{s}) &(\textit{mWh}) &time& (\textit{s}) & (\textit{mWh})& time\\
    \hline
        Temp./hum. & 5.55 & 0.79 &1y 4m&  2.46 & 0.35& 2y 2m\\
        IR-based & 5.12 & 0.73 & N/A& 2.19 & 0.31&N/A\\
        Magnetic & 5.10 & 0.73 & N/A& 2.18 & 0.31&N/A\\
    \hline
  \end{tabular}
  }
\end{center}
\caption{Energy consumption of sensors.  The time and energy reported is the time and energy taken to wake up, join the WiFi network, perform a reading, and  report the reading to the cloud. 
For \TOOL, reporting the reading to the cloud involved performing all \TOOL checks and then performing a transaction to send the reading to the \TOOL server (a remote server comparable to the Particle cloud).
Battery lifetimes assume one sensor reading is reported on average per an hour.
\label{tab:energyconsumption}}
\vspace{-2em}
\end{table}

Our Particle Photons
wake up, read the sensor, and then go to deep sleep.
The humidity/temperature sensors are read on average once an hour
while the other sensors wake up the Particle Photon on demand.  
}
\myparagraph{Particle Cloud---Energy and Privacy}
We evaluated \TOOL against the Particle cloud framework as the Particle cloud framework has an easily available SDK that has been used to develop many commercial IoT products.  
%Table~\ref{tab:energyconsumption} summarizes the
%energy consumption.
We configured a Particle Photon to read a
humidity/temperature sensor and powered it with 3 AA
batteries.  When using the Particle cloud, it
takes at least 5.55 seconds to wake up, connect, publish value, and
go back to sleep.  The total energy consumed for the wake-up time
of 5.55 seconds is 0.79mWh.
Assuming that it wakes up every hour to do one
measurement and goes back to sleep, the total energy consumed is 1.17mWh
each hour for deep sleep plus reporting a measurement.  
Three Energizer AA Lithium batteries provide approximately 13.5Wh and thus,
could support measurements for 1 year and 4 months.  When using 
Fidelius server, it takes only 2.46 seconds to complete the same
measurement cycle. Hence, its hourly power consumption is 0.73mWh,
and it could support measurements up to 2 years 2 months.

\mycomment{
\begin{table}[th]
	\begin{tabular}{cc}
		\begin{minipage}{.5\linewidth}
		\centering
		\footnotesize
		  \begin{tabular}{| c | c |}
			\hline
				\multicolumn{2}{| c |}{\javacode{Particle.publish()}}\\
			\hline
				Argument Length & Payload\\
			\hline
				8 & 34\\
				16 & 34\\
				32 & 50\\
				64 & 82\\
				128 & 146\\
				256 & 210\\
			\hline
		  \end{tabular}
		\end{minipage} &

		\begin{minipage}{.5\linewidth}
		\centering
		\footnotesize
		  \begin{tabular}{| c | c |}
			\hline
				\multicolumn{2}{| c |}{\javacode{Particle.function()}}\\
			\hline
				Argument Length & Payload\\
			\hline
				8 & 34\\
				16 & 50\\
				32 & 66\\
				63 & 98\\
			\hline
		  \end{tabular}
		\end{minipage} 
	\end{tabular}
	\caption{Information leakage of \javacode{Particle.publish()} and \javacode{Particle.function()}.\label{tab:informationleakage}}
\end{table}}

%\mysubsubsection{Information Leakage}
The network trace shows that the Particle cloud 
leaks information about the argument lengths.
\mycomment{Table~\ref{tab:informationleakage} presents the results.}
The \javacode{publish()} method, which allows a device to publish results 
on the Particle cloud in a key-value fashion, sends different packet 
lengths for different argument lengths, e.g., a 16-character argument results in 
a 34-byte payload, a 32-character argument results in a 50-byte payload, etc.
The \javacode{function()} method, which allows devices to publish
C code functions on the Particle cloud, behaves in a similar way.
\mycomment{
e.g., a 16-character argument results in a 50-byte payload, a 32-character
argument results in a 66-byte payload, etc.
Moreover, the Particle cloud has knowledge of all requests and must be trusted.
}
For \TOOL, the network trace only shows a \code{getmsg} is always followed by a
\code{putmsg} request with uniformly-sized data blocks.
We randomized the wake-up time of our sensors that need
to give periodic updates---\ie temperature/humidity sensor.
Since every \TOOL request had the exact same traffic pattern, we were not able to determine the type of \TOOL request from the traffic.


\mycomment{
\begin{table}[!htb]
\centering
\footnotesize
\begin{tabular}{|c|c|c|c|}
\hline
	Operation & \begin{tabular}[c]{@{}c@{}}Total\\ Time\end{tabular} & 
	\begin{tabular}[c]{@{}c@{}}Network and\\ Server Delay\end{tabular} & 
	\begin{tabular}[c]{@{}c@{}}\TOOL \\ Client Delay\end{tabular} \\ \hline
	New Key-Value  & 43.96 ms & 26.40 ms & 17.57 ms \\ \hline
	Key-Value Update & 139.45 ms & 26.42 ms & 113.03 ms\\ \hline
\end{tabular}
\caption{\TOOL Evaluation Data on Raspberry Pi 1\label{tab:evalTab}}
\vspace{-2em}
\end{table}

\mysubsection{Microbenchmarks}\label{sec:microbench}
We evaluated \TOOL on several microbenchmarks.  
Table~\ref{tab:evalTab} presents the results:
the first row presents the results for 2 clients creating 4,000 new key-value pairs, and the second row the results for 
making 2 updates to them.
In each benchmark, the keys were arbitrated by a remote machine. 
No network failures were introduced during this evaluation.
The clients ran on outdated Raspberry Pi 1s that have a low
performance processor.
}
\mycomment{
Note that when the client is executed on a
laptop with a 2.5 GHz Core i5, 
the client delays drop to 1.14 ms and 3.24 ms for new key-value 
creation and key-value update, respectively.
Thus, the overhead of \TOOL is reasonable compared to the overall
network delay.
}

\mycomment{
% % http://www.tablesgenerator.com/
\begin{table}[]
\centering

\resizebox{.48\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|}
\hline

Operation & \begin{tabular}[c]{@{}c@{}}Total\\ Time\end{tabular} & \begin{tabular}[c]{@{}c@{}}Network and\\ Server Delay\end{tabular} & 
\begin{tabular}[c]{@{}c@{}}\TOOL \\ Client\\ Delay\end{tabular} & \begin{tabular}[c]{@{}c@{}}\TOOL \\ Client\\ Overhead\end{tabular} \\ \hline
\begin{tabular}[c]{@{}c@{}}New LAN\\ Key-Value\end{tabular} & 4.10ms & 3.80ms & 0.30ms & 7.27\% \\ \hline
\begin{tabular}[c]{@{}c@{}}New Remote\\ Key-Value\end{tabular}  & 37.61ms & 37.04ms & 0.58ms & 1.53\% \\ \hline
%\begin{tabular}[c]{@{}c@{}}New LAN \\ Transaction\\ Local Arbitrate\end{tabular} & 6.51ms & 4.13ms & 2.37ms & 36.45\% \\ \hline
\begin{tabular}[c]{@{}c@{}}New LAN \\ Transaction \end{tabular} & 5.18ms & 3.99ms & 1.19ms & 22.92\% \\ \hline
%\begin{tabular}[c]{@{}c@{}}New Remote\\  Transaction \\ Local Arbitrate\end{tabular}  & 39.95ms & 36.24ms & 3.71ms & 9.28\% \\ \hline
\begin{tabular}[c]{@{}c@{}}New Remote\\  Transaction \end{tabular} & 38.12ms & 36.17ms & 1.96ms & 5.13\% \\ \hline
\end{tabular}}
\caption{\TOOL Evaluation Data\label{tab:evalTab}}
\end{table}
}

%\mysubsection{Comparison to Path ORAM}\label{sec:pathoram}
\myparagraph{Path ORAM}
\mycomment{
\begin{table}[th]
  \centering
  \begin{center}
  { \footnotesize
  \begin{tabular}{| r | r | r | r | r | r |}
    \hline
        Blocks & \multicolumn{2}{| c |}{Total Time (\textit{s})} & 
        	\multicolumn{2}{| c |}{Time/Access (\textit{s})} & Factor\\  	
    \cline{2-5}
        & Path ORAM & \TOOL & Path ORAM & \TOOL &\\
    \hline
        63 & 45.67 & 10.59 & 0.72 & 0.17 & 4.3$\times$\\
        127 & 119.25 & 21.97 & 0.94 & 0.17 & 5.4$\times$\\
        255 & 294.03 & 43.85 & 1.15 & 0.17 & 6.7$\times$\\
        511 & 503.27 & 86.68 & 0.98 & 0.17 & 5.8$\times$\\
    \hline
  \end{tabular}
  }
  \end{center}
  \caption{Access times for different numbers of blocks.
  \label{tab:accesstimes}}
\vspace{-2em}
\end{table}

\begin{table}[th]
  \centering
  \begin{center}
  { \footnotesize
  \begin{tabular}{| r | r | r | r |}
    \hline
        Blocks & \multicolumn{2}{| c |}{Total Transmission (\textit{kB})} & Factor\\  	
    \cline{2-3}
        & Path ORAM & \TOOL &\\  	
    \hline
        63 & 4,296.58 & 175.21 & 24.5$\times$\\
        127 & 10,887.89 & 353.83 & 30.8$\times$\\
        255 & 25,796.25 & 710.50 & 36.3$\times$\\
        511 & 61,324.40 & 1,422.88 & 43.1$\times$\\
    \hline
  \end{tabular}
  }
  \end{center}
  \caption{Data transfer for different numbers of blocks.
  \label{tab:datatransmission}}
\vspace{-1em}
\end{table}
}

PyORAM, a Python implementation of the Path ORAM
algorithm~\cite{stefanov-ccs13b}.\footnote{
Path ORAM is one of the few cloud-based
oblivious storage system implementations that are publicly available~\cite{pyoram}.
Path ORAM assumes the weaker honest but curious adversarial model.
%PyORAM implements caching of the top-levels of the Path ORAM tree.
%PyORAM also keeps the position map in local storage and thus does not
%need to perform a separate network access to locate a block.
}
We tried to run PyORAM's Path ORAM on the Raspberry Pi as a client.
\mycomment{
Unfortunately, it could only support 7 blocks of data---it
crashed when more blocks were added.  Because of this, we used a
laptop with a 
2.5GHz Intel Core i5 and 8GB 
of RAM as a client instead. On this machine, PyORAM can be configured 
to cache the top 2 levels of the tree with a height of 8 and up to
511 blocks of data---we believe that real systems could
easily have this many keys.
}
%Table~\ref{tab:accesstimes} reports our experimental results that show
%access times.
The results show an increasing trend of time per access
for PyORAM as the tree height and number of blocks grow, while for \TOOL
time per access is always steady. For 255 blocks,
\emph{\TOOL was already 7$\times$ faster than PyORAM}---this  
difference is caused by the nature of PyORAM benchmark that is bandwidth 
limited.
%Table~\ref{tab:datatransmission} reports the average data
%transmissions of different numbers of blocks for both %PyORAM
%and \TOOL.  
As the tree height and number of blocks grow, the total
amount of transferred data also increases faster
than \TOOL---for 511 blocks, \emph{PyORAM transfers more than
43$\times$ the amount of data that \TOOL transfers.}

%of RAM as a client instead. On this machine, PyORAM can be configured 
%to cache the top 2 levels of the tree with a tree height of 8 and
%511 blocks of data---this was the largest number of blocks
%we could run on the system and we believe that real systems could
%easily have this many keys.  For \TOOL, each transaction performed one
%put.  PyORAM took on average 52.28 ms per write operation while \TOOL
%took on average 4.74 ms per operation. Thus, \emph{\TOOL was
%11.03$\times$ faster than PyORAM}---this huge difference is caused
%by the nature of PyORAM benchmark that is bandwidth limited, even
%for our small setup with 511 blocks of data and a tree-height of 8.

\mycomment{
\section{Discussion}
\label{sec:discussion}
Obviously, we make trade-offs in \TOOL's design. \TOOL
aims to provide privacy guarantees in the case that
an adversary has obtained complete control over the
cloud server: a malicious server.
In achieving this, \TOOL practically takes away the
server's ability to look into the stored data under
normal operational conditions, \eg to perform data
analytics.
Thus, the implication is twofold. First, \TOOL may not
be suitable for all IoT applications. However, it
can be effective for certain scenarios that do not
the server to comprehend the data, 
\eg when running a private application
on a public cloud service. \footnote{This application might be
running on the cloud to coordinate and communicate with
different entities (\eg IoT devices, smartphones, etc.).}
Second, data analytics can still be performed
using another machine that also has access to the
encryption keys used by the clients---practically
another client.
}

==> Securing Smart Home Edge Devices against Compromised Cloud Servers/intro.tex <==
\mysection{Introduction}\label{sec:intro}
\mycomment{
Smart home devices have received increasing attention due to their ability to
provide smart functionality include lights,
door openers, water flow sensors, smart meters, IP-enabled cameras, motion sensors, and
door locks. These devices can be easily attacked, leading to privacy leaks or even physical home damages~\cite{fernandes-oakland16}. Much work~\cite{vigilia, flowfence,he-sec18} has been done at various layers of the stack to protect such client-side applications and devices.
}

In contrast to extensive research on client-side smart home security, the security of the cloud servers
that control these client-side devices has received less attention from researchers.
%Compromising cloud servers has the potential to let attackers control
%and monitor smart home IoT devices \emph{at scale}.
This is particularly concerning---e.g., recent work shows that if an attacker can control enough high-wattage
IoT devices, the attacker can cause power grid
failures~\cite{powergrid1}.
Implementing attacks \emph{at scale} by compromising individual smart home devices is not
straightforward due to the sheer number of devices that must be hacked.  
%Although these client devices are far from hardened targets, hacking many of them at the same time is 
%hard---for example, many deployed
%smart home thermostats (such as Nest) do not have any open ports. 
%Furthermore, typical home networks place devices behind a NAT
%firewall, making them hard to attack from the Internet.
%Smart home apps and devices typically communicate through cloud servers, such as the SmartThings cloud or the Google Home cloud.  
Thus, compromising cloud servers can be a more practical
approach.  In fact, the year of 2018, alone, has seen a huge number of compromises to cloud servers, including those
operated by many well-known companies (\eg Facebook~\cite{facebook}, Marriott~\cite{marriott}, Sony~\cite{sony}, etc.)

\mycomment{
Such as
Facebook~\cite{facebook}, Marriott~\cite{marriott}, Sony~\cite{sony},
Panera~\cite{panera}, Ticketfly~\cite{ticketfly}, Quora~\cite{quora},
Newegg~\cite{newegg}, Rail Europe~\cite{raileurope}, British Airways~\cite{britishairways},
and Target~\cite{target}.
}

In addition to large-scale attacks on
physical infrastructures, there are other concerns with trusting the 
cloud: 
(1) \textit{Privacy:} Smart home devices collect a great deal of
information about  users~\cite{smarthomecollectinginfo1}.
%, which is sent to the cloud and users have limited knowledge or control of how it is used.
Private data can be leaked if a cloud server is compromised.
(2) \textit{Traffic Analysis:} 
%Even if the server itself is not
%compromised, 
It may be possible to learn information by
observing traffic patterns~\cite{princeton-spying-castle}.
For example, such an analysis could reveal that when the thermostat's
mode transitions (\eg from \textit{Home} to \textit{Away}), it always sends
a packet of a specific length~\cite{copos2016anybody}. 
By watching traffic, attackers could discover whether people are home.

\mycomment{
\myparagraph{Prior Work} 
%Prior work~\cite{feldman-dissertation} observes that just signing and encrypting updates is insufficient to protect clients against an untrusted server.  While signatures prevent an untrusted server from forging messages, the server can still attack clients by using existing  messages that have valid signatures.  
%For example, the server can send clients mixtures of old and new versions of data; replay old requests; drop updates; and send different clients different, inconsistent views of the data.  

Traditionally, Byzantine fault tolerance (BFT)~\cite{lamport-toplas82}
has been used in distributed system implementations to mitigate the
threat of equivocation and other forms of misbehavior.
Unfortunately, BFT systems are
costly because each function needs to be executed multiple times on
multiple servers and the servers should have independent 
implementations to avoid having common vulnerabilities.
Furthermore, the system cannot make progress if a quorum of servers is
unavailable.

Recent distributed file systems~\cite{sundr,cloudproof} have defended against malicious servers without requiring costly duplication by enforcing variants of a property called \emph{fork consistency}, which is the strongest consistency model possible without trusted online parties.  In fork consistency, clients share
their individual views of the order of operations by embedding the history they see in each operation they send. 
%If clients to whom the provider has equivocated see each others' operations, they will soon discover the provider's misbehavior. The provider can still \emph{fork} the clients into disjoint
%groups and only tell each client about operations by others in its group, but then it
%can never again show operations from one group to the members of another without
%being detected. Furthermore, if clients are occasionally able to exchange views of
%the history out-of-band, even a provider which forks the clients will not be able to
%cheat for long.

%SUNDR provides fork consistency by
%maintaining signed histories---the cloud server must keep a signed
%history indefinitely for clients that have not been contacted
%recently.  CloudProof~\cite{cloudproof} improves on fork consistency by having the data
%owner periodically request and audit all client data accesses. However, 
%consistency violations can only be detected at the next
%audit after they actually occur. Moreover, consistency violations may not be
%detected at all for clients that are offline during the audit.  Caelus~\cite{caelus}
%uses timing assumptions combined with a single auditor to provide
%consistency guarantees.  The auditing process introduces
%a single point of failure---if the auditor dies, the entire system
%halts.  

Although fork consistency systems can effectively detect server misbehavior, existing approaches suffer from three major 
drawbacks, making them unsuitable for IoT settings. 
First, existing systems can incur large
storage costs as they need to keep an unbounded history of operations
for the entire time a device goes to sleep to allow the device to verify
that the server has not misbehaved.  Second, none of
these systems prevents the server from learning what records clients
have accessed.
%---malicious servers could easily determine whether a
%home owner is present based on the records updated and/or accessed (\eg using the traffic analysis discussed above).
Third, challenges also arise due to network connectivity.  
In smart home systems, devices are sometimes powered by batteries and may not have sufficient energy to be continuously on the Internet.  
%Consider for
%example the Nest thermostat in which the user can set a heating and
%cooling schedule.  The Nest thermostat harvests power
%from control wires and stores this power in a rechargeable battery.  To
%conserve battery power, the Nest thermostat may disconnect from the
%network.   Network connectivity can be lost for long periods, and it is desirable for the app to be usable even when this happens.
%A related issue arises when Internet connectivity is lost.  A
%smartphone app on the same network should still be able to control
%smart home devices like a light bulb.  Indeed, the Nest thermostat, LiFX,
%SmartThings, and WeMo all support some form of local control.
\mycomment{
The CAP
theorem~\cite{captheorem}, a well-known result in distributed systems,
implies that if we want a smart home system to tolerate home
Internet outages, we must give up either consistency or availability.
In particular, a smart home system can
provide strong consistency by halting the system until connectivity is
restored, hurting usability, or strong availability by
providing weaker semantics for updates, sacrificing consistency and
security.   Finding a workable compromise between consistency and availability is a challenge in the design of smart home systems.
}}

\begin{figure}[!htb]
\vspace{-.5em}
\begin{center}
\includegraphics[scale=0.49]{figures/cloud}
\end{center}
\vspace{-1em}
\caption{System Overview\label{fig:overview}}
\vspace{-2em}
\end{figure}

%\subsection{Our Approach}
\myparagraph{Our Approach: \TOOL}
%Motivated by the weaknesses of prior work, 
%this paper presents \TOOL.
Motivated by these security and privacy concerns, this paper
presents \TOOL.
\TOOL provides consistency and security
to smart home devices even in the presence of compromised servers in realistic smart home environments that include 
the presence of intermittent network accesses.
Figure~\ref{fig:overview} presents an overview of the \TOOL system.
A \TOOL deployment consists of (1) an untrusted cloud-based server
that provides connectivity between clients, (2) any number of clients
that are smart home devices, and (3) any number of clients that are
smartphone apps.  Our server implementation is architected as a
FastCGI server that communicates with the Apache Web Server. 
We focus our work on providing a
secure \emph{key-value storage system} targeted at IoT applications.\footnote{
The Nest thermostat API
communicates data in JSON as a tree of key-value pairs that can be
easily stored using a key-value abstraction.  Similarly, Apple HomeKit
associates a set of properties and corresponding values with each
device.  %These characteristics are effectively keys and thus the
%HomeKit protocol can also be viewed as key-value
%based.
}
%~\cite{theodoblog}.}
While existing systems use adhoc protocols for communicating data, the standard
\emph{key-value abstraction} is powerful enough to subsume a
wide-range of adhoc protocols.
We do not impose special 
requirements on server hardware; instead, the \TOOL 
enforcement runs on \emph{each client device}. Clients communicate with the server; in the absence of Internet connectivity, they can also 
communicate with each other locally
to maintain functionality.\footnote{This is already supported in many smart home systems today such as LiFX and Hue light bulbs, WeMO outlets, and TP-Link outlets.}
This design is well matched for the smart-home environment where 
%(1) devices have increasingly large compute power, memory, and storage space and (2) %they 
devices are mutually connected in a local home network. 

\myparagraph{Contributions}
This paper makes the following contributions:
\squishlist
\item {\bf Secure Transactional Key-Value Store:}
  It presents a key-value store that provides strong
  security and privacy guarantees even if the server is malicious.
\item {\bf Local Control:} It presents an algorithm supporting local control of smart home devices
when  connectivity is lost.
\item {\bf Transactional Programming Model:}  It presents developers with a transactional model to abstract consistency and availability tradeoffs that arise from network partitions.
\item {\bf Evaluation:} 
%It evaluates the performance of \TOOL  using a test bed system with an app built on \TOOL
%  and 16 smart home class devices.  It presents energy
%  measurements, microbenchmarks, and comparisons with both
%  a commercial IoT cloud framework (Particle.io) and PyORAM~\cite{stefanov-ccs13b}, an ORAM-based oblivious storage implementation. 
Compared to Particle.io, \TOOL reduces more than \textbf{50\%} of the data communication time and increases battery lifetime by \textbf{2$\times$}. Compared to PyORAM,  \TOOL has \textbf{4-7$\times$} faster access times with \textbf{25-43$\times$} less data transferred. 
\squishend

%\todo{Random thought...  It would be conceptually possible to build a
%protocol checker/sniffer than dynamically checks that a given device doesn't try
%to leak keys or send data outside of the protocol...It would also be
%possible to build a protocol firewall that blocks all communication to
%IoT devices that doesn't follow the protocol...Both approaches would require knowing the key %%though...}


==> Securing Smart Home Edge Devices against Compromised Cloud Servers/kvstore.tex <==
\mysection{Transactional Key-Value Store}\label{sec:kvstore}

We next present the transactional key-value store.
\TOOL's transactional key-value store is built on top of its message passing layer.  It relies on the message passing layer to ensure that the transactional key-value store layer receives a consistent set of messages from the server.

\mysubsection{Transaction Operations}

We next present the set of operations the transactional key-value store supports:
\squishlist
\item {\bf Assigning an Arbitrator:}
Before a key can be used it must be created and
assigned an arbitrator using a method which creates a new key record. If the key already exists or if the creation
fails the client will be notified.  The arbitrator of each key
$\mathsf{k}$ is stored with a new key record, which records the device 
that arbitrates the key $\mathsf{k}$.

\item {\bf Updating Key-Value Pairs:}
Transactions update key-value pairs by using the \code{Put} function.
These updates are stored locally until the transaction is committed.

\item {\bf Looking up Keys:}
A transaction can retrieve the values that are paired with keys using
the \code{GetCommittedAtomic} or the \code{GetCommitted} functions.
Recall that accesses using the \code{GetCommittedAtomic} functions
ensure serializability and thus introduce guard conditions that must
be checked when committing the transaction.

\item{\bf Commiting Transactions:}
To commit a transaction, the client creates a transaction record.
A transaction record is a tuple\mycomment{,
$\tuple{\sserver, \stlocal, \id, \KV{}, \MYG{}}$} that is comprised of
the set $\KV{}$ of key-value pairs \mycomment{---a key-value pair is
$\tuple{k,v}$---}to be updated, the guard condition $\MYG{}$ that
consists of the set of key-value pairs to be validated before
committing the transaction, and the sequence number $\sserver$ of
the message that first contained the transaction record.  The
combination of the machine ID $\id$ that created the transaction
and the client's local transaction sequence number $\stlocal$ is used
to uniquely specify the transaction.

The client then attempts to send the record to the server or in the event of
a network failure tries to send the record to the arbitrator.
\TOOL returns a future that the client can use to check 
whether a transaction committed.

Once a transaction record has been created, the client code
attempts to send it to the server.  Recall that multiple clients might
make \putmsg requests to the server simultaneously. This can cause
the \putmsg requests to fail.  If this occurs, the client simply
retries sending the same transaction record.  Note that this merely
reattempts sending the record and does not retry the underlying
transaction.  Furthermore, there may be more records that need to be
sent than a message can fit, and thus clients may need to send
multiple messages to enqueue all pending record data into the queue.

In the event of a network failure, the client falls back to local
communication and sends transactions directly to the arbitrator if local
communication is possible.
\squishend

\mysubsection{Arbitrating Transactions}

As stated previously each key is arbitrated by a specific device to
support committing transactions even when server connectivity is lost.
An arbitrator commits a transaction by evaluating the guard condition
$\MYG{}$ of that transaction to verify that that transaction is
serializable. This allows transactions to be predicated on specific
key-value pairs from the current committed set of key-value pairs at
the time when the transaction was created. When a transaction is
arbitrated, if the transaction is not serializable, \ie at least one
of the $\tuple{k,v} \in \MYG{}$ is not contained in the current set of
committed key-value pairs, then all key-value updates in $\KV{}$ are
ignored and the transaction is aborted. Otherwise, the updates are
performed and the transaction is committed.

When a transaction arbitrator decides to commit a transaction, it
creates a commit record
\mycomment{$\tuple{\sserver, \arbLocalId, \tLocalId,\\ \KV{}}$} to record the
updates to key-value pairs.  A commit record contains the set $\KV{}$
of updated key-value pairs.  The record also contains the sequence
number $\sserver$ of the message that first contained the commit
record, the arbitrator's machine ID $\idarblocal$ and local
arbitration sequence number $\sarblocal$, and the pair of the machine ID
$\idtlocal$ and the local transaction sequence number $\stlocal$,
which together uniquely specifies the original transaction.  A $\commit$
record keeps track of the updated key-value pairs.  Thus, a $\commit$
record is live until every key-value pair in the commit record is overwritten by newer commits.

If an arbitrator decides to abort a transaction, it creates an abort
record \mycomment{$\tuple{\sserver,\arbLocalId, \tLocalId}$} to inform the client
that created the transaction that the transaction has not been
accepted.  The abort record contains the sequence number $\sserver$ of
the message that first contained the abort record, the arbitrator's
machine ID $\idarblocal$ and local arbitration sequence number
$\sarblocal$, and the machine ID $\idtlocal$ and the local transaction
sequence number $\stlocal$, which uniquely specifies the original
transaction.  Since abort records are used by the server to notify
the client that generated a transaction that the transaction aborted,
an abort record is live until the client that generated the
transaction has confirmed the receipt of the abort record by inserting
a message with a sequence number that is larger than the abort's
sequence number.

After arbitration, commits and aborts are sent to the server
so that clients may see them.  In the event of a network failure,
clients can request commits and aborts be passed locally.

Transaction records are processed by arbitrators in order of
$\sserver$.  Thus, a commit or abort for a transaction with $\sserver$
implies that all transactions with the same arbitrator as that
transaction (but with a smaller $\sserver$) have been arbitrated and
that the transaction record is no longer live.

\mysubsection{Processing Commit and Abort Records}

Abort records do not require any processing since their purpose is (1)
to mark a transaction record dead and (2) to allow clients to be
notified of aborted transactions.  Commit records are stored in a
temporary buffer and processed after all commit records from the new
messages have been extracted since they may be received out of order
and thus need to be sorted before they can be processed.

Clients can obtain the latest key-value pairs by requesting and
processing new messages from the server.  During the update process,
all pending commits, aborts, and transactions that have not been
enqueued to the server, or passed locally in the case of transactions,
are enqueued using the same method described above. If the server is
not reachable, then key-value pairs can be updated using local
communication by requesting all new commits and aborts directly from
the key's arbitrator.


\mysubsection{Handling Network Failures}

As a result of an ill-timed network failure during an attempt by a
client to enqueue a message that contains a transaction record,
a client could have successfully inserted a transaction record into
the queue but not received a response from the server.  If local
communication is not possible then the client will try to enqueue the
same transaction at a later time.  If a transaction
happens to be sent twice, the arbitrator will detect this by
comparing the transaction records' $\tLocalId$ tuple and ignore
the second copy.  If local communication occurs then there is a chance
that an arbitrator will see the same transaction record twice, once
from the server and once directly from the client.  As in the previous
case, the arbitrator will detect the duplication and ignore the second
copy.






\mycomment{
\mysubsection{Implementation}

Our implementation includes extra functionality including: (1) support
for transactions and key-value pairs of any
size, (2) commit compression that combines multiple commits to save
space, and (3) a presumed commit optimization.  This functionality is
described in Appendix~\ref{sec:opt}.% of the technical report~\cite{technicalreport}.
}








==> Securing Smart Home Edge Devices against Compromised Cloud Servers/makefile <==
LATEX := pdflatex -halt-on-error

.SUFFIXES : .tex .bbl .aux .eps .ps .dot .pdf

.tex.bbl:
	bibtex $*

.tex.aux:
	latex $*

%.eps: %.ps
	ps2epsi $< $@

%.ps: %.dot
	dot -Tps $< -o $@

%.pdf: %.dot
	dot -Tpdf $< -o $@

%.png: %.dot
	dot -Tpng $< -o $@

%.aux: %.tex
	$(LATEX) $<

# latex the paper (default)
new:	biblinks newpaper

# latex + bibtex the paper
bib:	bibpaper newpaper


biblinks: figures
	$(LATEX) paper.tex
	bibtex paper.aux
	$(LATEX) paper.tex

newpaper: figures biblinks
	$(LATEX) paper.tex

bibpaper: paper.aux paper.bbl
	latex paper.tex

spell:
	@for i in *.tex; \
	do if [ $$i != "paper.tex" ]; then aspell -c $$i -p ./spell.lst; fi;\
	done


total:
	pdflatex paper.tex
	bibtex paper.aux
	pdflatex paper.tex
	pdflatex paper.tex
	@echo ================================================================
	pdflatex paper.tex | grep -E 'arning|erfull'
	@echo ================================================================


figures: $(FIGURES)



clean:
	rm -f *.dvi *.log *.aux *.blg *.bbl *~
	rm -f paper.ps paper.pdf 


==> Securing Smart Home Edge Devices against Compromised Cloud Servers/opt.tex <==
\mysection{Implementation}\label{sec:opt}

Our implementation has extra functionality and
optimizations including
support for transactions of any size.

\myparagraph{Arbitrary Sized Key-Value Pairs and Transactions}
Our implementation supports key-value pairs of any size.  Our implementation does not require
individual commits and transactions fit in a single fixed-size message.
Our
implementation instead allows transactions and commits to be broken into 
parts.  Key-value data is broken into parts and span as
many records as needed.  Transactions 
and commits are pieced together from their parts to recover the key-value
data for commit and transaction processing.

\myparagraph{Transaction Speculation}

Recall that many IoT devices are only intermittently online to save power.  We
also expect that the cloud server would typically be reachable and
thus local communication would infrequently occur.  Thus our implementation supports
transaction speculation---an optimization that allows clients to
obtain key-value pairs from transactions before the transactions are
actually committed by the arbitrator.  This optimizes for the common
case and allow clients to provide a more interactive experience.

This optimization is implemented by examining the set of committed
key-value pairs and the set of pending-arbitration transactions to determine the
set of transaction commit decisions that the arbitrator will make assuming
that there are no locally communicated transactions.  Clients may 
use the speculative values as guard conditions for future
transactions.

\myparagraph{Commit Compression}
During arbitration many transactions that operate on the same
key-value pairs may be arbitrated together.
For example, this can happen when an arbitrator is offline for a period of
time and then pulls messages from the server. This may
cause some commits to contain key-value pairs that have been
overwritten by a newer commit processed in the same batch.
To avoid sending commit information that will immediately be
overwritten our implementation compresses several commits
into one or more larger commits.  Multiple updates to the same key-value
pair from multiple commits will be compressed to only a single
update with that single update being the update from the most recent
commit.  This new commit will be at most as large as the sum of the
sizes of commits it compresses but could be significantly smaller if
many commits updated the same keys. When a commit
becomes very large or a part of the commit has been sent, it will
no longer be compressed.

We also have a presumed commit optimization---if a
transaction with a later identifier is processed, early committed
transactions are presumed to have committed and the commit records can
be elided.  Thus, it is important to maintain constraints
on the relative ordering of commits and aborts---aborts must appear
at least as early as they did in the original order to ensure that they are not presumed to have committed.  If an abort
appears in the middle of a sequence of commits that is compressed, it
must be sent before the commits.

%Our implementation includes extra functionality including: (1) support
%for transactions and key-value pairs of any
%size, (2) commit compression that combines multiple commits to save
%space, and (3) a presumed commit optimization.  This functionality is
%described in Appendix~\ref{sec:opt}.% of the technical report~\cite{technicalreport}.




==> Securing Smart Home Edge Devices against Compromised Cloud Servers/overview.tex <==
\mysection{Overview}\label{sec:overview}

\begin{figure}[!htb]
\vspace{-.5em}
\begin{center}
\includegraphics[scale=0.43]{figures/BlockChain}
\end{center}
\vspace{-1.4em}
\caption{Message Chain\label{fig:messagechain}}
\vspace{-1.em}
\end{figure}

\TOOL uses a message chain to provide secure, totally ordered
communications between clients.  Since the server is not trusted, the
clients must be able to locally verify the integrity of the message
chain.  Therefore, each message in the chain has a fixed size and
contains a unique sequence number, a keyed-hash message authentication
code (HMAC) of the previous message in the chain, and a set of
records.  Finally, each message contains an HMAC of itself.  This
ensures that the message cannot be modified.  The HMACs are generated
using a key known only to the clients to ensure that the server cannot forge
messages.  When a message is transported between clients, it is always
encrypted using the transport key.  Together, this ensures that the
server cannot know the contents of messages nor can it modify them.

\paragraph{Message Truncation and Refreshing Records}
A simple message chain would eventually consume all memory on the
devices and server.  Thus, \TOOL is designed such that the last $n$
messages in the chain have enough information to reconstruct the state
of the key value store.  This enable \TOOL to truncate the message
chain.  An important secondary benefit of truncating the message chain
is that the amount of work that a client that goes to sleep and then
wakes after a long period of time must perform is bounded by $n$.

Records in the key-value store can potentially be long-lived.  Thus a
consequence of our design choice is that such records must be
reinserted into the message chain (or refreshed) before they are
truncated.


==> Securing Smart Home Edge Devices against Compromised Cloud Servers/proof.tex <==
\mysection{Security of Message Passing}\label{sec:proof}

A second security concern is ensuring that the server cannot corrupt
communications between clients.  HMACs ensure the integrity of
individual messages, but do not prevent the server from sending old
message, accepting multiple messages with the same sequence number,
etc.  We thus prove a theorem that if two devices receive the same
message, then all previous messages they have received are consistent.


\mycomment{\begin{theorem}
Suppose that there is a transitive closure set $\mathsf{\mathscr{S}}$
of clients, at sequence number $\mathsf{n}$. Then there is some
total sequence $\mathsf{T}$ of length $\mathsf{n}$ such that every
client~$\mathsf{C}$ in $\mathsf{\mathscr{S}}$ sees a partial sequence
$\mathsf{P_C}$ consistent with $\mathsf{T}$.
\end{theorem}

\begin{proof}
See Appendix~\ref{sec:proof}.
\end{proof}}


In this Section, we present the guarantees provided by the message
passing layer.  We start by presenting several definitions and then prove several properties.  

\begin{defn}[Equality]
Two messages $\mathsf{t}$ and $\mathsf{u}$ are equal if their
$\mathsf{s}$ and $\mathsf{Dat_t}$ are equal.
\end{defn}

\begin{defn}[Parent]
A parent of a message $\mathsf{t}$ is the message $\mathsf{p_t}$, 
unique by the correctness of HMACs in $\mathsf{Dat_t}$, such that 
$\mathsf{hmac_p(t) = hmac_c(p_t)}$.
\end{defn}

\begin{defn}[Chain]
A chain of messages with length $\mathsf{n \ge 1}$ is a message
sequence $\mathsf{R = (r_s, r_{s+1}, ..., r_{s+n-1})}$ such that for
every sequence number $\mathsf{s < k \le s+n-1}$, $\mathsf{r_k}$ has
sequence number $\mathsf{k}$ and its parent is $\mathsf{r_{k-1}}$.
\end{defn}

\begin{defn}[Partial sequence]
A partial sequence $\mathsf{P}$ is a sequence of messages, no two with
the same sequence number, that can be divided into disjoint chains.
\end{defn}

\begin{defn}[Total sequence]
A total sequence $\mathsf{T =}$ $\mathsf{(t_1, t_2, ..., t_n)}$ with
length $\mathsf{n}$ is a chain of messages that starts at $\mathsf{s =
  1}$.
\end{defn}

\begin{defn}[Path]
The path of a message $\mathsf{t}$ is the total sequence whose last
message is $\mathsf{t}$. The uniqueness of a path follows from the
uniqueness of a parent.
\end{defn}

\begin{defn}[Consistency]
A partial sequence $\mathsf{P}$ is consistent with a total sequence
$\mathsf{T}$ of length $\mathsf{n}$ if for every message $\mathsf{p
  \in P}$ with sequence number $\mathsf{s_p \leq n}$, $\mathsf{t_{s_p} = p}$. This
implies that $\mathsf{\{p \in P | s_p \le n\}}$ is a partial sequence
of $\mathsf{T}$.
\end{defn}

\begin{defn}[Transitive closure]
The transitive closure set at sequence number $\mathsf{s_n}$ is a set
$\mathsf{\mathscr{S}}$ of clients comprising a connected component of
an undirected graph, where two clients are connected by an edge if
they both received the same message $\mathsf{t}$ with sequence number
$\mathsf{s_t > s_n}$.
\end{defn}


\begin{prop}
\label{prop:parentmessage}
Every client~$\mathsf{J}$ who sends a message $\mathsf{t}$ has parent
$\mathsf{p_t}$ as its latest stored message and $\mathsf{s_t =
  s_{p_t} + 1}$.
\end{prop}
\begin{proof} True by construction, because client~$J$ sets 
$\mathsf{hmac_p(t) = hmac_c(p_t)}$ and $\mathsf{s_t = }$
  $\mathsf{s_{p_t + 1}}$ when a message is sent.
\end{proof}

\begin{prop} 
\label{prop:rejectedmessage}
If a rejected message record is added to the queue at
sequence number $\mathsf{s}$, the record will remain in the queue
until every client has seen it.
\end{prop}
\begin{proof}
Every record $\de{}$ remains in the queue until it
reaches the tail, and is refreshed by the next sender $\mathsf{J}$ at
that time until every client
has sent a message with a sequence number greater than
$\mathsf{s}$. Because every client who sends a message with
sequence number $\mathsf{s'}$ has a copy of the entire queue at
$\mathsf{s' - 1}$, this client will have seen the message at
$\mathsf{s}$.
\end{proof}

\begin{figure}[!htb]
\resizebox{.5\textwidth}{!}{
  \centering
      \xymatrix{ & & L \\
\dots \ar[r] & q \ar[dr]_{J} \ar[r]^{K} & l_1 \ar[r] & l_2 \ar[r] & \dots \ar[r] & m \ar[r] & \dots \ar[r] & l_n = u \\
& & r_1 \ar[r] & r_2 \ar[r] & \dots \ar[r] & r_m = t \\
& & R
\save "2,3"."2,8"*+\frm{^\}}
\save "3,3"."3,6"*+\frm{_\}}
\restore
\restore
      }
      }
\caption{By \textbf{Lemma~\ref{lem:twomessages}}, receiving both $t$
  and $u$ here is impossible.\label{fig:fork}}
\end{figure}


\begin{lem}
\label{lem:twomessages}
If two messages, $\mathsf{t}$ and $\mathsf{u}$, such that $\mathsf{s_t \le s_u}$
are received by a client~$\mathsf{C}$ without any clients reporting errors,
then $\mathsf{t}$ is in the path of $\mathsf{u}$.
\end{lem}
\begin{proof}
Assume that there are some pairs of messages $\mathsf{(t,u)}$ that
violate this lemma for some client~$\mathsf{C}$.  Take a specific pair
$\mathsf{(t,u)}$ and client~$\mathsf{C}$ such that $\mathsf{s_u}$ is
minimized, and $\mathsf{s_t}$ is maximized for this choice of
$\mathsf{s_u}$. We will show that client~$\mathsf{C}$ cannot receive both
$\mathsf{t}$ and $\mathsf{u}$ without some client throwing an error.

Clearly client~$\mathsf{C}$ will throw an error if $\mathsf{s_t = s_u}$. So
$\mathsf{s_t < s_u}$. Additionally, if client~$\mathsf{C}$ receives
$\mathsf{u}$ before $\mathsf{t}$, this will cause it to throw an
error, so $\mathsf{t}$ must be received before $\mathsf{u}$. We will prove
that an error occurs upon receipt of $\mathsf{u}$.

Let $\mathsf{r_1}$ be the earliest member of the path of $\mathsf{t}$
that is not in the path of $\mathsf{u}$, and let $\mathsf{q}$ be its
parent. Message $\mathsf{q}$, the last common ancestor of $\mathsf{t}$
and $\mathsf{u}$, must exist, since all clients and the server were
initialized with the same state. Let $\mathsf{l_1}$ be the successor
of $\mathsf{q}$ that is in the path of $\mathsf{u}$; we know
$\mathsf{l_1 \neq r_1}$. Let $\mathsf{R = (r_1, r_2, \dots, r_{|R|} =
  t)}$ be the distinct portion of the path of $\mathsf{t}$, and
similarly let $\mathsf{L}$ be the distinct portion of the path of
$\mathsf{u}$.

Let $\mathsf{J}$ be the client who sent $\mathsf{r_1}$; that is, such
that $\mathsf{{id_{self}}_J = GetMacID(r_1)}$, and $\mathsf{K}$ be the
client who sent $\mathsf{l_1}$. Because no client can send two
messages with the same sequence number, and $\mathsf{s_{r_1} = s_{l_1}
  = s_q + 1}$, $\mathsf{J \neq K}$.

We next prove the two propositions that we will use to complete this
proof.

\begin{prop} 
\label{prop:bothmessages}
No client sends both a message in $\mathsf{(r_2,...,t)}$ and a message
in $\mathsf{(l_2,...,u)}$.
\end{prop}

\begin{proof}
To send a message $\mathsf{p}$ that is the parent of some other
message, one must have received the parent of $\mathsf{p}$. Since
$\mathsf{u}$ is the message with smallest sequence number received by
any client that violates Lemma~\ref{lem:twomessages}, no client can
receive both a message in $\mathsf{r}$ and a message in $\mathsf{l}$.
\end{proof}

\begin{prop} 
\label{prop:seqnumb}
Client~$\mathsf{C}$ does not receive any message with a sequence number
strictly between $\mathsf{s_t}$ and $\mathsf{s_u}$.
\end{prop}

\begin{proof}
If there were such a message with sequence number smaller than
$\mathsf{s_u}$, it would contradict the assumption that $\mathsf{u}$
is the message with the least sequence number that violates
Lemma~\ref{lem:twomessages}.
\end{proof}

We continue the proof of Lemma~\ref{lem:twomessages}.  There are two cases:
\begin{itemize}
\item Case 1: Client~$\mathsf{J}$ did not send a message in
  $\mathsf{L}$. Define $\mathsf{s_{t_J}}$ to be the greatest sequence
  number of the messages that client $\mathsf{J}$ sent in the path of
  message $\mathsf{t}$.  Define $\mathsf{s_{q_J}}$ and
  $\mathsf{s_{u_J}}$ similarly.  We then have $\mathsf{s_{t_J} >
    s_{q_J} = s_{u_J}}$.
\begin{itemize}
\item Case 1.1: Client~$\mathsf{C}$ never calls $\code{ValidateLastMessages()}$
  between receiving $\mathsf{t}$ and receiving $\mathsf{u}$; by
  Proposition~\ref{prop:seqnumb} this can only happen if $\mathsf{s_t
    = s_u - 1}$. Since $\mathsf{t}$ is not the parent of $\mathsf{u}$,
  $\mathsf{hmac_p(u) \neq hmac_c(t)}$, causing client~$\mathsf{C}$ to throw
  an error.
\item Case 1.2: Case 1.1 does not occur; therefore, client~$\mathsf{C}$ calls
  $\code{ValidateLastMessages()}$ at some point between receiving
  $\mathsf{t}$ and $\mathsf{u}$.  The latest sequence number of
  client~$\mathsf{J}$ decreases during this time, which means client~$\mathsf{C}$
  throws an error in the $\code{ValidateLastMessages()}$ function.
\end{itemize}
\item Case 2: Client~$\mathsf{J}$ sent at least one message in
  $\mathsf{L}$. Call the first one $\mathsf{m}$. We know that
  $\mathsf{s_m > s_{r_1}}$, since $\mathsf{J \neq K}$ and $\mathsf{m
  \neq l_1}$.  Since the current sequence number for $\mathsf{J}$ can
  only increase, client~$\mathsf{J}$ must send the message
  $\mathsf{r_1}$ before the message $\mathsf{m}$.  Let $\mathsf{X =
    (r_1 = x_1, \dots, x_n)}$ be the list of messages client~$\mathsf{J}$
  sends starting with $\mathsf{r_1}$ and ending immediately before $m$; clearly
  these all have sequence number $\mathsf{\geq s_q + 1}$.
\begin{itemize}
\item Case 2.1: Some message in $\mathsf{X}$ was accepted by the
  server. Therefore, before sending $\mathsf{m}$, client~$\mathsf{J}$'s value
  in $\code{lastmessage}$ for its own latest sequence number would be
  greater than $\mathsf{s_{q_J}}$. If there is a sequence of messages
  with contiguous sequence numbers that client~$\mathsf{J}$ receives
  between $\mathsf{r_1}$ and $\mathsf{m}$ (switching from the
  $\mathsf{R}$ chain to the $\mathsf{L}$ chain), client~$\mathsf{J}$
  throws an error for a similar reason as Case 1.1. Otherwise, when
  preparing to send $\mathsf{m}$, client~$\mathsf{J}$ would have
  received an update of its own latest sequence number as at most
  $\mathsf{s_{q_J}}$. Client~$\mathsf{J}$ throws an error before
  sending $\mathsf{p}$, because its own latest sequence number
  decreases.

\item Case 2.2: All messages in $\mathsf{X}$ were rejected by the
  server, making $\mathsf{m}$ the first message of client~$\mathsf{J}$
  that is accepted after $\mathsf{r_1}$.

We will prove that client~$\mathsf{C}$ sees $\mathsf{r_1}$ by
contradiction. Assume not. Then $\mathsf{(r_2, ..., t)}$ must have at
least $\currqsize_C \geq 2$ messages for $\mathsf{r_1}$ to fall off
the end of the queue (note that by Proposition~\ref{prop:seqnumb}
client~$\mathsf{C}$ cannot receive the next message after
$t$). Consider the sender of $\mathsf{r_3}$ and call it $\mathsf{H}$.
$\mathsf{H \neq J}$ by Proposition~\ref{prop:bothmessages} and the
existence of $\mathsf{m}$.  Since $\mathsf{H \neq J}$, then by
Proposition~\ref{prop:bothmessages} it could not also have sent a
message in $\mathsf{(l_2,..., u)}$. Therefore, $\mathsf{s_{u_H} < s_q
  + 2 = s_{t_H}}$, so upon receipt of $\mathsf{u}$, client~$\mathsf{C}$ will
throw an error by the decrease in a last sequence number similar to
Case 1, a contradiction.

Now that we know that client~$\mathsf{C}$ must receive
message~$\mathsf{r_1}$, note that client~$\mathsf{C}$ receives
$\mathsf{u}$ immediately after $\mathsf{t}$ by
Proposition~\ref{prop:seqnumb}. Therefore, client~$\mathsf{C}$ could not have
seen a message after $\mathsf{t}$ with sequence number less than
$\mathsf{s_m}$. In the $\code{AttemptSendRecord()}$ function,
client~$\mathsf{J}$ adds a rejected message record that contains sequence
number $\mathsf{s}$ and its machine ID to record the rejected
messages.  Hence, for every $\mathsf{i}$, $\mathsf{1 \leq i < |X|}$,
the rejected message $\mathsf{x_i}$ from client~$\mathsf{J}$ will be
recorded. Since all the rejected message records that store the rejected
messages will also be seen when $\mathsf{u}$ is received, and
client~$\mathsf{C}$ sees $\mathsf{r_1}$, ${r_1}$ will be recorded as a
rejected message.  When client~$\mathsf{C}$ receives $\mathsf{u}$, it will
throw an error due to previously having received a message that was
marked as rejected.
\end{itemize}
\end{itemize}
\end{proof}

\begin{lem} 
\label{lem:pathmessages}
If there are two messages $\mathsf{t}$ and $\mathsf{u}$, with
$\mathsf{s_t \leq s_u}$, such that $\mathsf{t}$ is in the path of
$\mathsf{u}$, then for any message $\mathsf{p}$ with $\mathsf{s_p \leq
  s_t}$, iff $\mathsf{p}$ is in the path of $\mathsf{t}$, it is in the
path of $\mathsf{u}$.
\end{lem}

\begin{proof}
If $\mathsf{s_t = s_u}$ or $\mathsf{s_p = s_t}$, then we are done,
because the two relevant messages are the same. If they are different
messages, then:
\begin{itemize}
\item Reverse direction: The definition of $\mathsf{t}$ being in the
  path of $\mathsf{u}$ is the existence of a message sequence
  $\mathsf{(\dots, t, \dots, u)}$ such that each message except
  $\mathsf{u}$ is the parent of the succeeding message.  The path of
  $\mathsf{u}$ must contain some message with sequence number
  $\mathsf{s_p}$; because $\mathsf{p}$ is in the path of $\mathsf{u}$,
  this message is $\mathsf{p}$ itself. The path of $\mathsf{t}$ is
  then the prefix of this path ending at $\mathsf{t}$, which clearly
  contains $\mathsf{p}$.

\item Forward direction: The path of $\mathsf{t}$ is a substring of
  the path of $\mathsf{u}$, so if the path of $\mathsf{t}$ contains
  $\mathsf{p}$, so does the path of $\mathsf{u}$.
\end{itemize}
\end{proof}

\begin{theorem}
Suppose that there is a transitive closure set $\mathsf{\mathscr{S}}$
of clients, at sequence number $\mathsf{n}$. Then there is some
total sequence $\mathsf{T}$ of length $\mathsf{n}$ such that every
client~$\mathsf{C}$ in $\mathsf{\mathscr{S}}$ sees a partial sequence
$\mathsf{P_C}$ consistent with $\mathsf{T}$.
\end{theorem}

\begin{proof}
The definition of consistency of $\mathsf{P_C}$ with $\mathsf{T}$ is
that every message $\mathsf{p \in P_C}$ with sequence number
$\mathsf{s_p \le n}$ is equal to the message with that sequence number in
$\mathsf{T}$. Let $\mathsf{C_1}$ be some client in the transitive
closure set, with partial sequence $\mathsf{P_{C_1}}$, and let
$\mathsf{u}$ be some message with $\mathsf{s_u > n}$ that
$\mathsf{C_1}$ shares with another client. Then let $\mathsf{T}$ be
the portion of the path of $\mathsf{u}$ ending at sequence number
$\mathsf{n}$ and $\mathsf{t}$ be the message at that sequence
number. Clearly, by Lemma~\ref{lem:twomessages}, $\mathsf{P_{C_1}}$ is
consistent with $\mathsf{T}$. We will show that, for every other
client $\mathsf{D}$ with partial sequence $\mathsf{P_D}$,
$\mathsf{P_D}$ has some message whose path includes
$\mathsf{t}$. Because $\mathsf{D}$ is in the transitive closure, there
is a sequence of clients $\mathsf{\mathscr{C} = (C_1, C_2, ..., D)}$
from $\mathsf{C_1}$ to $\mathsf{D}$, where each shares an edge with
the next.  We prove by induction that $\mathsf{P_D}$ has a message
whose path includes $\mathsf{t}$.
\begin{itemize}
\item Base case: $\mathsf{P_{C_1}}$ includes $\mathsf{u}$, whose path
  includes $\mathsf{t}$.

\item Inductive step: Each client in $\mathsf{\mathscr{C}}$ has a
  partial sequence with a message that includes $\mathsf{t}$ if the
  previous client does. Suppose $\mathsf{P_{C_k}}$ has a message
  $\mathsf{w}$ with a path that includes $\mathsf{t}$, and shares
  message $\mathsf{x}$ with $\mathsf{P_{C_{k+1}}}$ such that
  $\mathsf{s_x > n}$. By Lemma~\ref{lem:twomessages}, $\mathsf{w}$
  or $\mathsf{x}$, whichever has the least sequence number, is in the
  path of the other, and therefore by Lemma~\ref{lem:pathmessages},
  $\mathsf{t}$ is in the path of $\mathsf{x}$.

\item Let $\mathsf{z}$ be the message of $\mathsf{D}$ whose path
  includes $\mathsf{t}$.  By Lemma~\ref{lem:twomessages}, every
  message in $\mathsf{P_D}$ with sequence number smaller than
  $\mathsf{s_w}$ is in the path of $\mathsf{z}$. Since $\mathsf{t}$ is
  in the path of $\mathsf{z}$, every message in $\mathsf{P_D}$ with
  smaller sequence number than $\mathsf{s_t = n}$ is in
  $\mathsf{T}$.  Therefore, $\mathsf{P_D}$ is consistent with
  $\mathsf{T}$.
\end{itemize}
\end{proof}


==> Securing Smart Home Edge Devices against Compromised Cloud Servers/pseudocode.tex <==
\newpage
\mysection{Key Value Store Pseudocode}\label{sec:pseudocode}
\begin{figure}[!htb]
  \footnotesize
  \begin{algorithmic}[1]
    \Function{ValidateandUpdate}{Messages[] $\newmsgs$}
      \If{$|\newmsgs| = 0$}
        \State{\Return{}}
      \EndIf
      \State{$\code{ResetQueueSizeCounter}()$}
      \State{Check that first message has a sequence number that is $\geq \seqnum$.}
      \ForAll{$\fullmsg$ in $\newmsgs$}
        \State{Decrypt $\encpayload$ to obtain $\payload$.}
        \State{Validate that $\seqnume = \seqnum$.}
        \State{$\code{Validate}(\payload)$.}
        \State{$\code{IncrementQueueSizeCounter}()$}
      \EndFor

      \If{Gap exists between $\localqueue$ and $\newmsgs$}
      \State{$\code{ValidateQueueSizeCorrect}(|\newmsgs|)$}
      \State{$\code{ValidateLastMessages}()$}
      \EndIf
    \If{we sent a message that is still unresolved}
    \State{Create reject message entry for message}
    \EndIf
    \State{Update $\qsize$ using $\currqsize$ and resize $\localqueue$.}
      \State{$\code{UpdateLastMessages}()$}
      \State{Add decrypted $\newmsgs$ to $\localqueue$.}
      \State{Update $\currseqnum$.}
      \State{$\code{processKVStore}()$}
    \EndFunction
  \end{algorithmic}
\caption{\label{fig:validateupdate}Validate and Update Procedure}
\end{figure}

% Individual Message Validation
\begin{figure}[!htb]
  \footnotesize
  \begin{algorithmic}[1]
    \Function{Validate}{$\payload$}
      \State{Validate $\hmacc=HMAC(\payload)$.}
      \State{Validate $\hmacp=HMAC(\payload_{p})$.}
      \State{$\code{processLastMsg}(\tuple{\id,\seqnum})$}
      \ForAll{$\de{}$ in $\DE{}$}
        \If{$\de{}$ is a $\lastmsg$}
          \State{$\code{processLastMsg}(\de{})$}
        \ElsIf{$\de{}$ is a $\queuestate$}
          \State{$\code{processQueueStatus}(\de{}, \seqnume)$}
        \ElsIf{$\de{}$ is $\rejmsg$}
          \State{$\code{processRejectedMsg}(\de{})$}
        \Else
          \State{$\code{processKVStoreRecord}(\de{})$}
        \EndIf
      \EndFor
    \EndFunction
  \end{algorithmic}
\caption{\label{fig:validatemsg}Validate Individual Message}
\end{figure}

% Record Handlers
\begin{figure}[!htb]
  \footnotesize
  \begin{algorithmic}[1]
    \Function{processLastMsg}{$\tuple{\id, \seqnum'}$}
      \If{$\localid=\id \wedge \seqnum'$ is marked as unresolved}
      \State{Mark $\seqnum'$ as accepted and no longer unresolved}
      \EndIf
      \State{lastmsg[$\id$]:=$\seqnum'$}
    \EndFunction

    \Function{processQueueStatus}{$\tuple{n}, \seqnume$}
      \State{$\currqsize:=n$}
      \State{$\code{SetQueueSizeCounter}(\seqnume, n)$}
    \EndFunction

    \Function{processRejectedMsg}{$\rme$}
      \State{Validate that $\forall \tuple{\seqnum, \payload} \in \localqueue, \mathsf{s_{low}} \leq \seqnume \leq \mathsf{s_{high}} \Rightarrow \id_{\mathsf{rme}} \neq \id$ }
    \EndFunction
  \end{algorithmic}
\caption{\label{fig:messagehandler}Record Handlers}
\end{figure}

\newpage
\begin{figure}[!htb]
  \footnotesize
  \begin{algorithmic}[1]
    \Function{UpdateLastMessages}{}
    \ForAll{$\id$ in machines}
    \If{lastmsg[$\id$] $\neq 0$}
    \State{committedlastmsg[$\id$] = lastmsg[$\id$]}
    \EndIf
    \EndFor
    \EndFunction\\
    \Function{ValidateLastMessages}{}
    \ForAll{$\id$ in machines}
    \State{Validate lastmsg[$\id$] $\neq 0$}
    \State{Validate lastmsg[$\id$] $\geq$ committedlastmsg[$\id$]}
    \EndFor
    \State{Validate lastmsg[$\localid$] = our last accepted message}
    \EndFunction
    \end{algorithmic}
\caption{Last Message Validation\label{fig:lastmessage}}
\end{figure}

%\begin{figure}[!htb]
\begin{figure}[!htb]
  \footnotesize
  \begin{algorithmic}[1]
    % \Function{ResetQueueSizeCounter}{$\seqnume, n$}
    \Function{ResetQueueSizeCounter}{}
      \State{$\mathsf{counterReset} := \true$}
    \EndFunction\\

    \Function{SetQueueSizeCounter}{$\seqnume, n$}
      \If{$\mathsf{counterReset}$}
        \State{$\mathsf{counterReset} := \false$}
        \State{$\mathsf{expectedSize} := min(\seqnume, n)$}
        \State{$\mathsf{currentMaxSize} := n$}
      \EndIf
    \EndFunction\\

    \Function{IncrementQueueSizeCounter}{}
      \If{$\mathsf{expectedSize} < \mathsf{currentMaxSize}$}
        \State{$\mathsf{expectedSize} := \mathsf{expectedSize} + 1$}
      \EndIf      
    \EndFunction\\

    \Function{ValidateQueueSizeCorrect}{$n$}
      \State{Validate that $n = \mathsf{expectedSize}$}
    \EndFunction
  \end{algorithmic}
\caption{\label{fig:expectedmsgs}Compute Expected Number of Messages}
\end{figure}

\newpage
\begin{figure}[!htb]
  \footnotesize
  \begin{algorithmic}[1]
    \Function{SendRecord}{$\de{}$}
    \If{there is a message whose status is unresolved}
    \If{$\neg \code{ResendPastMessage}()$}
    \State{\Return{Had Server Timeout}}
    \EndIf
    \EndIf
    \State{forceresize:=$\false$}
    \State{$\DE{}:=\emptyset$}
    \If{$\code{ResizeThresholdReached()} \vee$ forceresize}\label{resize}
    \State{Calculate new queue size and resize threshold.}
    \State{$\DE{}:=\{$ New Resize Queue Record$\}$}
    \EndIf
    \State{$\DE{}:=\DE{} \cup $Generate $\rejmsg$ record for rejected msg list.}
    \If{$\lnot \code{MandatoryRefresh}(\DE{}) \land$ Not Resizing}
    \State{forceresize := $\true$}
    \State{$\DE{} := \emptyset$}
    \State{\Goto{resize}}
    \EndIf
    \If{$\code{HasSpace}(\DE{}, \de{})$}
    \State{$\DE{} := \DE{} \cup \{\de{}\}$}
    \EndIf
    \State{$\DE{} := \DE{} \cup$ Live records in other old messages that fit.}
    \State{$p:=\mathsf{\tuple{\currseqnum, \localid, \hmacp, \DE{} }}$.}
    \State{Send to server using: $\putmsg(\mathsf{\tuple{\currseqnum, E(\tuple{p, HMAC(p)}) }})$\label{putmessage}}
    \If{Server accepted message}
    \State{$\code{ValidateandUpdate}$($\mathsf{\tuple{\currseqnum, E(\tuple{p, HMAC(p)}) }}$)}
    \State{\Return{$\de{} \in \DE{}$}}
    \ElsIf{Server rejected message}
    \State{Add $\seqnum$ to rejected message list.\label{createrejectedmessage}}
    \State{$\code{ValidateandUpdate}$(Messages returned by server)\label{processservermessage}}
    \State{\Return{$\false$}}
    \ElsIf{Server never responds after timeout\label{networkissuestart}}
    \State{Mark message status as unresolved}
    \State{\Return{Had Server Timeout}\label{networkissueend}}
    \EndIf
    \EndFunction\\
\end{algorithmic}
\caption{\label{fig:sendrecord}Method to Send Record}
\end{figure}

\begin{figure}[!htb]
\begin{algorithmic}
  \footnotesize
    \Function{ResendPastMessage}{} 
      \State{Resend previous $\msg$ using: $\putmsg(\mathsf{\tuple{\currseqnum, E(\tuple{p, HMAC(p)}) }})$}
      \If{Server accepted message}
        % \State{Unmark message resent message $\seqnum$ as unresolved message}
        \State{$\code{ValidateandUpdate}(\mathsf{\tuple{\currseqnum, E(\tuple{p, HMAC(p)}) }})$}
        \State{\Return{$\true$}}
      \ElsIf{Server rejected message}
        % \State{Unmark message resent message $\seqnum$ as unresolved message}
        \If{Resent $\msg$ not in response $\land$ no $\lastmsg$ with same $\seqnume$ and $\id$ as $\msg$}
          \State{Add resent $\msg$ to rejected message list}
        \EndIf
        \State{$\code{ValidateandUpdate}$(Messages returned by server)}
        \State{\Return{$\true$}}
      \ElsIf{Server never responds after timeout}
        \State{\Return{Had Server Timeout}}
      \EndIf
    \EndFunction\\

    \Function{MandatoryRefresh}{$\DE{return}$}
    \If{oldest slot is unused}
    \State{\Return $\true$}
    \EndIf
    \State{Find the oldest $\tuple{s, \payload}$ in $\localqueue$}
    \ForAll{$e \in \DE{}$ that are alive}
    \If{$\lnot \code{HasSpace}(\DE{return}, e)$}
    \State{\Goto{endPosition}}
    \EndIf
    \State{$\DE{return} := \DE{return} \cup \{e\}$}
    \EndFor
    \State{\Return if oldest message had all live records refreshed\label{endPosition}}
    \EndFunction
\end{algorithmic}
\caption{\label{fig:sendrecordhelpers}Helper Methods to Send Record}
\end{figure}

\newpage
% API
\begin{figure}[!htb]
  \footnotesize
  \begin{algorithmic}[1]
    \Function{StartTransaction}{}
      \State{$\tbuild := \tuple{\seqtlocal, \emptyset, \emptyset}$}
      \State{$\seqtlocal := \seqtlocal + 1$}
    \EndFunction\\

    \Function{CommitTransaction}{}
      \State{$\transaction := \code{GenerateTransaction}(\tbuild)$}
      \State{$\PendingTransact.\code{add}(\transaction)$}
      \State{$\code{DoCommunication}()$}
    \EndFunction\\

    \Function{CreateNewKV}{$k, \id$}
      \If{Key $k$ does not already exist}
        \State{\Return{$\code{SendRecord}(\tuple{k,\id})$}}
      \EndIf
      \State{\Return{Already Has Key $k$}}
    \EndFunction\\
    
    \Function{Update}{}
      \State{$\mathsf{newMsgs} :=$ Get new messages from server using $\getmsg$}
      \If{Had Server Timeout}
        \ForAll{$\id \in$ Known arbitrators}
          \State{$\code{SendLocally}$($null, \id$)}
        \EndFor
        \State{\Return{}}
      \EndIf
      \State{$\code{ValidateandUpdate}(\mathsf{newMsgs})$}
      \State{$\code{DoCommunication}()$}
    \EndFunction\\

    \Function{Put}{$k,v$}
      \State{$\code{CheckHasSameArbitrator}(k, \KV{\tbuild} \cup \MYG{\tbuild})$}
      \State{$\tbuild := \tuple{\stlocaltbuild, \KV{\tbuild} \cup \{\tuple{k,v}\}, \MYG{\tbuild}}$}
    \EndFunction\\

    \Function{GetCommitted}{$k$}
      \State{\Return $\committed[k]$}
    \EndFunction\\

%    \Function{GetSpeculative}{$k$}
%      \State{\Return $\speculated[k]$}
%    \EndFunction\\

    \Function{GetCommittedAtomic}{$k$}
      \State{$\code{CheckHasSameArbitrator}(k, \KV{\tbuild} \cup \MYG{\tbuild})$}
      \State{$\MYG{\tbuild}:=\MYG{\tbuild}\cup \{\tuple{k,\committed[k]}\}$}
      \State{$\tbuild := \tuple{\stlocaltbuild, \KV{\tbuild}, \MYG{\tbuild}}$}
      \State{\Return $\committed[k]$}
    \EndFunction

%    \Function{GetSpeculativeAtomic}{$k$}
%      \State{$\code{CheckHasSameArbitrator}(k, \KV{\tbuild} \cup \G{\tbuild})$}
%      \State{$\G{\tbuild}:=\G{\tbuild}\cup \{\tuple{k,\speculated[k]}\}$}
%      \State{$\tbuild := \tuple{\stlocaltbuild, \KV{\tbuild}, \G{\tbuild}}$}
%      \State{\Return $\speculated[k]$}
%    \EndFunction
  \end{algorithmic}
\caption{\label{fig:clientapi}Client Public API}
\end{figure}

\newpage
% Communication
\begin{figure}[!htb]
  \footnotesize
  \begin{algorithmic}[1]
    \Function{ReceiveLocally}{$\tuple{\transaction, \slastseen}$}
      \If{$\transaction \neq null \land $ Has not seen $\transaction$ before}
        \State{$\NewArb := \code{Arbitrate}(\{\transaction\})$}
        \State{$\PendingArbitration.\code{addAll}(\NewArb)$}
        \State{$\de{} := \NewArb.\code{getFront}()$}
        \If{$\de{}$ is a commit}
          \State{$\tuple{\sserver,\arbLocalId, \tLocalId, \KV{}} := \de{}$}
          \State{Update $\committed$ with $\KV{}$}
        \EndIf
      \EndIf
      \State{$\ArbSet := $ all live $\commit$ and $\abort$ where $\idarblocal= \localid$}
      \State{\Return{$\{\de{}|\de{} \in \ArbSet \land \slastseen < \sarblocal\}$}}
    \EndFunction\\

    \Function{SendLocally}{$\tuple{\sserver, \stlocal, \id, \KV{}, \MYG{}}, \idrec$}
      \State{$\LDat := \tuple{\tuple{\sserver, \stlocal, \id, \KV{}, \MYG{}}$, last $\sarblocal$ seen from $\id$ $}$}
      \State{Send $\LDat$ to $\idrec$ via \code{ReceiveLocally}}
      \State{$\newArbitration :=$ Returned $\{\de{}\}$ from \code{ReceiveLocally}}
      \If{Cannot Communicate Locally with $\id\lor$ Had Failure}
        \State{\Return{$\false$}}
      \EndIf
      \ForAll{$\de{} \in \newArbitration$}
        \State{$\code{processKVStoreRecord}(\de{})$}
      \EndFor
      \State{$\code{processKVStore()}$}
      \State{\Return{$\true$}}
    \EndFunction
  \end{algorithmic}
\caption{\label{fig:localcommunication}Local Communication Helper Functions}
  \end{figure}
  
\begin{figure}[!htb]
  \footnotesize
  \begin{algorithmic}[1]

    \Function{DoCommunication}{}
      \While{$|\PendingTransact| > 0 \lor |\PendingArbitration| > 0$}
        \If{$|\PendingArbitration| > 0$}
          \State{$\de{} := \PendingArbitration.\code{getFront}()$}
        \ElsIf{$|\PendingTransact| > 0$}
          \State{$\de{} := \PendingTransact.\code{getFront}()$}
        \EndIf            
        \State{Update $\sserver$ of $\de{}$ to $\seqnume$ of new message}
        \State{$\didSend:=\code{SendRecord}(\de{})$}

        \If{$\didSend$}
          \State{//Remove from appropriate list}
          \State{$\PendingArbitration.\code{remove}(\de{})$}
          \State{$\PendingTransact.\code{remove}(\de{})$}
        \ElsIf{Had Server Timeout}
          \ForAll{$\de{} \in \PendingTransact$} \label{haderror}
            \If{$\lnot$ $\code{SendLocally}(\de{}, $arbitrator $\id$ of $\de{})$}
              \State{//Stop sending to preserve ordering.}
              \State{Break}
            \Else
              \State{$\PendingTransact.\code{remove}(\de{})$}
            \EndIf
          \EndFor
          \State{Break}  
        \EndIf
      \EndWhile
    \EndFunction
  \end{algorithmic}
\caption{\label{fig:uppercommunication}Key-Value Store Communication Functions}
\end{figure}

\newpage
% Record Handlers
\begin{figure}[!htb]
  \footnotesize
  \begin{algorithmic}[1]

    % \Function{processAbort}{$\tuple{\sserver,\arbLocalId, \tLocalId}$}
    \Function{processAbort}{$\abort$}
      \State{//No Action must be taken here}
    \EndFunction\\

    \Function{processCommit}{$\commit$}
      \If{Client not seen $\commit$ before }
        \State{$\UnprocessedCom:=\UnprocessedCom \cup \{\commit\}$}
      \EndIf
    \EndFunction\\

    \Function{processTransaction}{$\transaction$}
      \If{Client not seen $\transaction$ before and is the arbitrator}
        \State{$\UnprocessedTran:=\UnprocessedTran \cup \{\transaction\}$}
      \EndIf
    \EndFunction\\

    \Function{processNewKey}{$\tuple{\mathsf{k}, \id}$}
      \If{$\id = \localid$}
        \State{Add self to be arbitrator for $k$}
      \EndIf
    \EndFunction\\

    \Function{processKVStoreRecord}{$\de{}$}
      \If{$\de{}$ is a $\abort$}
        \State{$\code{processAbort}(\de{})$}
      \ElsIf{$\de{}$ is a $\commit$}
        % \State{$\code{processCommit}(\de{}, \seqnume)$}
        \State{$\code{processCommit}(\de{})$}
      \ElsIf{$\de{}$ is $\transaction$}
        \State{$\code{processTransaction}(\de{})$}    
      \ElsIf{$\de{}$ is $\newkey$}
        \State{$\code{processNewKey}(\de{})$}   
      \EndIf    
    \EndFunction
  \end{algorithmic}
\caption{\label{fig:messagehandlerUpper}Key-Value Store Record Handlers}
\end{figure}

% Processing
\begin{figure}[!htb]
  \footnotesize
  \begin{algorithmic}[1]

    \Function{Arbitrate}{$Transactions[] T$}   
      \State{$\ArbRecs := []$}
      \State{$\committedTmp := \committed$}
      \ForAll{$\tuple{s_s, s_l, \id, \KV{}, \MYG{}} \in T,$ not arbitrated on $\land \id = \localid$}
        \If{$\forall \tuple{k,v} \in \MYG{}, \committedTmp[k] = v$}
          \State{$\ArbRecs.\code{add}(\code{GenCommit}(s_s, s_l, \id, \KV{}))$}
          \State{Update $\committedTmp$ with $\KV{}$}
        \Else
          \State{$\ArbRecs.\code{add}(\code{GenAbort}(s_s, s_l, \id))$}
        \EndIf
      \EndFor
      \State{\Return{$\ArbRecs$}}
    \EndFunction\\

%    \Function{Speculate}{}   
%      \State{$\speculated := \committed$}
%      \State{$\UnarbTSet:=$ all live transactions in $\localqueue$}
%      \State{$\UnarbTList:= \UnarbTSet$ sorted by $\sserver$}
%      \State{$\UnarbTList.\code{addAll}(\PendingTransact)$}
%      \ForAll{$\tuple{s_s, s_l, \id, \KV{}, \G{}} \in \UnarbTList$}
%        \If{$\forall \tuple{k,v} \in \G{}, \speculated[k] = v$}
%          \State{Update $\speculated$ with $\KV{}$}
%        \EndIf
%      \EndFor
%    \EndFunction\\


    \Function{processKVStore}{}
      \State{$\NewArb := \code{Arbitrate}(\UnprocessedTran$ sorted by $\sserver$)}
      \State{$\PendingArbitration.\code{addAll}(\NewArb)$}
      \State{$\UnprocessedCom := \UnprocessedCom \cup \{\de{} | \de{} \in \NewArb \land \de{} $is a $\commit \}$}
      \State{$\CList := \UnprocessedCom$ sorted by $\arbLocalId$}     
      \ForAll{$\tuple{\sserver,\arbLocalId, \tLocalId,\KV{}}\in \CList$}
         \State{Update $\committed$ with $\KV{}$}
      \EndFor
%      \State{$\code{Speculate}$}
      \State{$\UnprocessedTran := \UnprocessedCom := \emptyset$}
    \EndFunction
  \end{algorithmic}
\caption{\label{fig:upperprocessing}Transaction Processing}
\end{figure}


==> Securing Smart Home Edge Devices against Compromised Cloud Servers/rw.tex <==
\mysection{Related Work}\label{sec:related}

\mycomment{
Denning et al.~\cite{denning-cacm13}
made the first attempt to identify emergent threats to smart homes due
to the use of IoT devices. Recent work
discusses these threats in more
concrete contexts, for example, by demonstrating scenarios in which
hackers can weaken home security by compromising these devices~\cite{fernandes-oakland16}.
}
\mycomment{
There are two main categories of work in current smart home security
research, focused primarily on 
\emph{devices}~\cite{fisher-15,hesseldahl-15,ur-hups13}
and \emph{protocols}~\cite{fouladi-blackhat13, lomas-15,fernandes-oakland16},
respectively.}
\mycomment{
Work on devices includes the MyQ garage system that can
be used as a surveillance tool to inform burglars when the house is
possibly empty, the Honeywell Tuxedo touch controller that has
authentication bypass bugs and cross-site request forgery
flaws~\cite{fisher-15,hesseldahl-15}, as well as compact florescent
lamps that can induce seizures in epileptic
users~\cite{oluwafemi-laser13} and problems in the access control of the Philips Hue lighting system and the Kwikset door lock~\cite{ur-hups13}.
}

\mycomment{
A study on the access control of the
Philips Hue lighting system and the Kwikset door lock found that each
system provides a siloed access control system that fails to enable
essential use cases such as sharing smart devices with other users
like children and temporary workers~\cite{ur-hups13}. 
}
\mycomment{
On protocols, studies found
various flaws in the Zigbee and Z-Wave protocol
implementations~\cite{fouladi-blackhat13, lomas-15} as well as design
flaws in their programming frameworks~\cite{fernandes-oakland16}.  
A study from Veracode~\cite{veracode-15} on several smart home hubs
found that the SmartThings hub had an open telnet debugging interface
that can be exploited, while Fernandes et
al.~\cite{fernandes-oakland16} discovered framework design flaws in
the SmartThings platform.}

Oblivious RAM techniques, first proposed by Goldreich and
Ostrovsky~\cite{obliviousram}, seek to provide RAM~\cite{wang-ccs15,
  ren-usenixsecurity15, % wang-ccs14, wang-ccs14b,liu-oakland15
  stefanov-ccs13b, %dautrich-usenixsecurity14, maas-ccs13,
  stefanov-ndss12, liu-asplos15} or cloud
storage~\cite{stefanov-ccs13, stefanov-oakland13, %stefanov-ndss13,
  soled-onetwork15} in which the data access patterns
are independent of the computation and thus no
information can be extracted from the locations accessed.
Many
oblivious storage algorithms~\cite{obliviousram, stefanov-ccs13b} assume that
only one device can access the storage and that adversary is merely
honest but curious.  While some work does support multiple
clients~\cite{multiclient} or stronger adversarial
models~\cite{integrityverification}, these approaches assume that the
clients have limited local storage and thus incur bandwidth and/or latency overheads
for each access.

Much previous work on oblivious storage is
unsuitable for our scenario because: (1) it assumes an
honest, but curious adversary, and (2) it does not support multiple
clients accessing shared state.  Some recent work has removed the
single client limitation~\cite{multiclient} and supports stronger
adversarial models~\cite{integrityverification}.  However, most
oblivious RAM techniques incur extra overheads (e.g., latency or bandwidth)
for 
accesses to storage due to a fundamental limitation as a result of
the assumption that clients only have a small amount of storage.
Moreover, existing systems are not designed to support updates to
persistent state when connectivity has been lost and thus cannot
support local device control.

\mycomment{
There is a large body of work on building network systems that can
make communication unobservable
on untrusted infrastructures. Mix networks~\cite{
%  berthold-pet02, chaum-cacm81, danezis-oakland03, gulcu-ndss96,
  kesdogan-ih98, blond-sigcomm15, blond-sigcomm13} were used by the
 private messaging systems to shuffle messages before
delivering them to recipients.
Mailbox systems
techniques~\cite{hooff-sosp15, angel-osdi16, %borisov-pets15,
%cooper-oakland95, corrigan-gibbs-oakland15,kissner-acns04,
borisov-pets16, lazar-osdi16} provide security for messages
retrieved from mailboxes kept at third-party servers.  These
techniques are orthogonal.
}



==> Securing Smart Home Edge Devices against Compromised Cloud Servers/security.tex <==
\mysection{Privacy}\label{sec:security}

\TOOL provides both privacy and security.
The size of network packets or the records accessed can leak information about a computation.
\TOOL is designed to minimize the information leak by smart home devices.   We first discuss the privacy properties of \TOOL.

\begin{defn}[Privacy]
Let\\
{\footnotesize
\begin{equation*}\begin{split}\vec{x} := \tuple{\getmsg(i),\putmsg(\tuple{i, E(D_i)}),..., \getmsg(i+N-1),\\ \putmsg(\tuple{i+N-1, E(D_{i+N-1})})}
\end{split}\end{equation*}}
\end{defn}
denote a sequential data sequence of length $N$ from a single client.
We say that \TOOL is secure if for any two data request sequences
$\vec{x}$ and $\vec{y}$ of the same length, their request sequences
are computationally indistinguishable to the server.

We do not attempt to hide information that may be revealed through timing,
including the interleavings of requests from different clients.  We
thus prove that \TOOL is oblivious for a single client.  The proof can
be easily extended to executions of multiple clients that share an
interleaving schedule.

To prove the security of \TOOL, let $\vec{x}$ be an access sequence of
size $N$.  In the absence of a resize, the server sees the following
sequence of requests:\vspace{-.4em}

{\footnotesize \begin{equation*}\begin{split}\tuple{\getmsg(i),\putmsg(\tuple{i, E(D_i)})...,\getmsg(i+N-1), \\ \putmsg(\tuple{i+N-1, E(D_{i+N-1})})}\end{split}\end{equation*}}\vspace{-.8em}

Any two sequences of requests length $N$ that start at the same
sequence number $i$ will use the same sequence numbers.
While they will contain different encrypted data, the sequence
of encrypted messages sent by the \putmsg request is
computationally indistinguishable by the definition of encryption.
Note that different requests with the same data will produce entirely
different encrypted messages since no two AES blocks contain the
same counter value.


==> Securing Smart Home Edge Devices against Compromised Cloud Servers/technical.tex <==
%\mysection{Message Passing Layer}\label{sec:messagepassing}
\mysection{The \TOOL System}
\label{sec:example}

\mycomment{
%\mysubsection{Example}\label{sec:running-example}
%\myparagraph{Example}
As a running example, consider a smart thermostat such as a Nest, Honeywell, or Ecobee.
\mycomment{
Smart thermostats contain several sensors to determine the current
temperature and whether anyone is home in order to enable power saving functionality. Smart thermostats typically
include a smartphone app that  
allows users to control the current state of the thermostat and to
easily set heating and cooling schedules.


\begin{figure}[!htbp]
\vspace{-1.em}
\begin{lstlisting}[xleftmargin=3.0ex]
public TransactionStatus changeMode (Thermostat t,
    Mode newMode) {
  table.startTransaction();
  table.put(t.getModeKey(), newMode);
  return table.commitTransaction();
}
\end{lstlisting}\vspace{-1.em}
\caption{Code to set the Thermostat Mode\label{fig:modeset}}
\vspace{-1.em}
\end{figure}
}
In \TOOL, device functionalities are mapped to key-value pairs.  For example, thermostat apps support setting the mode of the thermostat to one of
four possible modes (OFF, COOL, HEAT, or RANGE).  The mode of a thermostat might be mapped to a mode key in the key-value store.  
To change the thermostat's operating mode, the smartphone app performs a transaction that updates the value corresponding to the thermostat's mode key.  For example, to turn the thermostat to the cooling (\ie COOL) mode, the transaction would update the mode key's value to COOL.
%\emph{cooling}.
The thermostat's operating mode then changes when it receives notification that the transaction has committed a change to the value corresponding to its mode key.  Similarly, other functionalities of the thermostat would be controlled by other key-value pairs, \eg high and low temperature setpoint.
}

\mycomment{
Figure~\ref{fig:modeset} presents example \TOOL code 
for the \javacode{changeMode} method, which sets the thermostat 
mode.
The \javacode{table} field references the key-value store.  The
\javacode{startTransaction} method call creates a new transaction.  The call to the \javacode{put} method updates a key-value pair; it stores the update in the local copy of the
table and does not forward the changes to the cloud server or
thermostat device.

Finally, the call to the \javacode{commitTransaction} method attempts to commit the
transaction.  If the cloud server is accessible,
the \javacode{commitTransaction} method sends an encrypted copy of the update to the
cloud server.
}

%\mysubsection{Design}\label{sec:design}
A key challenge in the design of \TOOL is how to handle the wide-range of
possible malicious behaviors from the server  while at the same time
support local control during Internet outages as well as intermittent availability of power-constrained devices.
To separate the concerns of 
handling malicious behaviors and implementing the key-value-store functionalities,
we architected \TOOL as two layers:
%\squishcount
%\item 
(1) a message passing layer that guarantees
consistent message delivery in the presence of  malicious
servers.  This layer handles all issues related
to malicious behaviors and does not implement any key-value-store functionalities; and
%\item 
(2) a transactional key-value store built on top of the
message passing layer.
%Unlike existing transactional key-value stores that assume connectivity is always maintained, 
%\TOOL's key-value store layer handles \emph{local communication} when server
%connectivity is lost.
%\countend
The app code runs on top of these two layers in each client---app developers can use the \TOOL API library in their code. On smart home devices, this code is the device controller code.  On smartphones, this is the actual app code. 

\mycomment{
Recall that \TOOL is architected as a key-value store built on top of a message passing layer.  We begin our presentation of \TOOL with the 
message passing layer. The key-value store layer (presented in Section~\ref{sec:kvstore}) uses the message passing layer to send data between clients via the cloud server.  
Data from the key-value store is stored in records that are part of the messages.   
Conceptually, the functionality of the message passing algorithm is simple: the server algorithm maintains a queue of all messages that are currently in use; 
the client algorithm supports (1) sending messages to the server
queue and (2) requesting a copy of the new messages in the current queue.  In addition to forwarding messages between clients, the server stores enough state so that new or long-absent clients can completely reconstruct the key-value store using the state in the server's queue.

The complexity in the algorithm arises in ensuring that compromised or otherwise malicious
servers do not violate the following correctness properties:
(1)  all clients receive a consistent set of messages, (2)  the server delivers all messages that it acknowledges, and
(3)  the server cannot forge messages or replay old messages.  The client algorithm detects and
signals an error if the server violates these properties.
}

\mysubsection{Message Passing Layer}\label{sec:message-passing}
Conceptually, the functionality of the message passing algorithm is simple: the server algorithm maintains a queue of all messages that are currently in use; 
the client algorithm supports (1) sending messages to the server
queue and (2) requesting a copy of the new messages in the current queue.  In addition to forwarding messages between clients, the server stores enough state so that new or long-absent clients can completely reconstruct the key-value store using the state in the server's queue.

\begin{figure}[!htb]
\begin{center}
\includegraphics[scale=0.43]{figures/BlockChain}
\end{center}
\vspace{-.5em}
\caption{Message Chain\label{fig:messagechain}}
\vspace{-1em}
\end{figure}

The \TOOL message passing layer uses a message chain to totally order
communications between clients that are sent via the cloud server.  Figure~\ref{fig:messagechain}
presents the structure of the message chain.  Each message in the
chain has a fixed size and contains (1) a globally unique sequence number, which is used to reference and order messages; (2) a
keyed-hash message authentication code (HMAC) of the previous message
in the chain, which is used to ensure the integrity of chain; and (3) a set of records, which can contain either data from the key-value store layer or control information that is needed to thwart attacks---we insert as much data as possible until the entire message reaches a certain fixed size specified through the \TOOL API.  Finally, each message contains an
HMAC of itself, which ensures that the message cannot be modified.
The HMACs are generated using a key known only to the clients to
ensure that the server cannot forge messages.  When a message is
transported between clients, it is always encrypted using the
transport key.  Together, this ensures that the server cannot know the
contents of messages nor can it modify 
them.\footnote{
Although the entire process might seem heavy for IoT devices that have limited resources, our evaluation energy consumption suggests that \TOOL can still perform efficiently (see Section~\ref{sec:eval}).}

\mycomment{
A \naive message chain would eventually consume all memory on the
devices and server.  Thus, \TOOL is designed such that the last $n$
messages in the chain have enough information to reconstruct the state
of the key-value store.  This enables the server to truncate the message
chain.  An important secondary benefit of truncating the message chain
is that the amount of work a client must perform when it 
wakes up after a long sleep is bounded by $n$.

Records in the key-value store can potentially still be in use (or \emph{live}) once they reach the end of the chain.  Thus, a
consequence of our design choice is that \TOOL must reinsert (or refresh) such records into the message chain before they are
truncated.  Section~\ref{sec:mpsend} provides details about how \TOOL determines whether a record is still live.
}

\myparagraph{Server Algorithm}
\mycomment{
The server algorithm implements
a shared, fixed-size message queue where clients can (1) insert new
messages and (2) read the contents of existing messages.  It is
important to note that the server is not trusted to correctly execute
this algorithm---clients will detect if the server incorrectly
executes the server algorithm.  However, if the server does not
correctly execute the server-side algorithm, it can prevent
transactions from committing.
}
The server maintains a queue of the last $n$ messages it has received.  Each message has a fixed-size encrypted block for which the server does not have the decryption key and a plain text sequence number $\seqnum$.
The server algorithm supports two requests: 
(1) \putmsg: add a new message\footnote{The server could first authenticate participating clients to avoid amplification attacks. However, this is out of the scope of this paper.} and 
(2) \getmsg: request messages that are currently
in the queue.  
Before adding a new message, it checks that its sequence number $\seqnum$ is one
greater than the previous sequence number.  If not, it sends a
rejection message back to the client that contains all messages in the
queue with a sequence number that is greater than or equal to
$\seqnum$.   Note that the clients must verify that the server correctly assigns these sequence numbers as we do not trust the server.
If a client detects that the key-value store state does not fit in the current queue, it can request that the server changes the size of the queue.
If a partial message is received, e.g., due to a network failure, the
server ignores the partial message.  If 
queue is full when a new message arrives, the server drops the oldest
message.  The client algorithm is responsible for ensuring that the information in the oldest message has been moved to a newer message before the message is dropped. 
A request for messages in the queue contains a sequence number $\seqnum$ that is one larger than the most recent message the client has received.  When the
server receives this request, it sends all messages
in its queue with sequence numbers that are equal or larger than
$\seqnum$ such that the client now has a up-to-date copy of the message chain.

\myparagraph{Client Algorithm}
\mycomment{$\msg = \mathsf{\tuple{s, E(Dat_s)}}$}
Clients communicates by sending and receiving messages through the server.
\mycomment{
A message $\msg$ consists of the sequence number $s$ and the encrypted
message body $\mathsf{E(Dat_s)}$.  The message body $\mathsf{Dat_s}$ consists of the sequence number $\seqnume$, the machine
ID $\id$ of the sender, the HMAC $\mathsf{hmac_p}$ from the previous
message, the set $\DE{}$ of records that contain the contents of the
message, and the HMAC $\mathsf{hmac_c}$ of the current message.
Messages have two copies of the sequence number as the server needs
access to the sequence number and the clients need a copy that they
can authenticate.  }
Our implementation uses the CTR mode of AES to encrypt messages.  A unique counter value
is sent to the server along with the message.  Clients share two
secrets that allow them to authenticate and encrypt messages: a
message authentic key 
%$k_{\text{hmac}}$ 
and a message encryption key. These are not known to the server.
%$k_{\text{enc}}$.  
%The server does not have access to these secrets.
%\todo{IT IS WORTH MENTIONING THAT THE SYSTEM ONLY CONSIDERS A BAD/MALICIOUS SERVER, NOT A BAD CLIENT; ALSO ALTHOUGH THE ENCRYPTION IS KIND OF HEAVY, IT IS ACCEPTABLE.}

\mycomment{
Our presentation of the client algorithm is structured as follows.
Section~\ref{sec:recvalidation} presents the
validation checks that clients perform when they receive messages.
Section~\ref{sec:mpsend} presents
the algorithm clients use to send messages.
}

When the message passing layer receives new messages from the server
(or they are created locally), the client decrypts and validates the
messages.  Records in messages at the message passing layer are used to both communicate
information for the key-value store layer and to thwart 
attacks that a malicious server may otherwise
perform.  
The proof in the technical report~\cite{technicalreport} shows that these checks suffice to thwart all server attacks: 
(1) \textit{Message Chain Integrity:}
To ensure the integrity of messages, after
decrypting a message the client
compares: computed HMAC against the stored
HMAC, $\seqnum$ from the server against $\seqnum$ in the message, and the HMAC of the current message against the HMAC of the message immediately proceeding
it, if present, in the queue. These are used to ensure that the server has not
manipulated the message chain.
(2) \textit{Detecting Dropped Messages:}
A malicious server could potentially acknowledge a message from a
client and then silently drop the message while a client is offline,
replacing it with a message with the same sequence number from another
client. To ensure that clients always detect
such dropped messages, the client algorithm uses {\it last message
records} to track the last message sent by itself and other clients so
that it can detect whether the server has dropped messages.  A last
message record consists of a
machine ID 
%$\id$ 
and the sequence number 
%$\seqnume$ 
of the last
message sent by that machine.  Last message records are only 
inserted if the most recent message from
a given machine ID is about to be evicted from the queue. 
(3) \textit{Detecting Reused Rejected Messages:}
The client algorithm uses {\it rejected message records} to detect if
the server attempts to use a rejected message.  A rejected message
record consists of the machine ID 
$\id$ 
of the
client that sent the rejected messages, the lowest sequence number
$\mathsf{s_{low}}$ 
and highest sequence number 
$\mathsf{s_{high}}$ 
of
the range of rejected messages, and the sequence number
%$\mathsf{s_{record}}$ 
of the first message that contained the rejected
message record.
To prevent this attack, each client verifies that each message in the
queue that has a sequence number that falls within the range of 
$\mathsf{s_{low}}$ and $\mathsf{s_{high}}$ has a machine ID $\id$ that 
is not equal to $\id$. 
The algorithm keeps a rejected message record 
live until all clients have seen it (as implicitly acknowledged by sending 
a newer message).\footnote{Since \TOOL does not keep the entire message chain, 
the server could temporarily fork the message chain and then move clients
from one fork to another if the client is offline for a sufficiently
long time such that all the messages the client has seen have been
evicted from the message chain. In the other fork, the server could
could send dropped or rejected messages.}
(4) \textit{Detecting Missing Messages:}
A malicious server could also attempt to send fewer messages than the
queue currently holds by omitting the oldest messages (noting that the 
message chain integrity checks prevent dropping messages in the middle).  
This would cause clients to compute the
key-value store state using an incomplete set of messages.
To prevent this, \TOOL uses {\it queue size record} to
store the current maximum capacity of the message queue and enables
clients to compute how many messages they should have received 
to validate that the correct number of messages was received.  

The message passing layer sends a message and performs the following bookkeeping tasks:
(1) \textit{Determine Which Records Must be Refreshed:}
If a record
$\de{}$ is live (the system is still using the information
they contain) then it must be refreshed by reinserting the record
into the queue before the message with that record leaves the queue.
A record $\de{}$ is dead iff one of the following conditions is true:
(i) a refreshed version of $\de{}$ is present in the 
queue,\footnote{A resize check is performed first to check if the number of messages
with records which are live in the queue exceeds a randomized resize threshold.
If so, a new queue size is calculated and a new queue size record
with the new size is inserted into the message.}
(ii) $\de{}$ is a queue size record and there is a newer queue size record,
(iii) item $\de{}$ is a rejected message record and all clients
have seen it as proven by having inserted a message into 
the queue with a $\seqnum$ that is greater than the $\seqnum$ of $\de{}$, or
(iv) $\de{}$ is a last message record and a client with the same $\id$ has inserted a 
newer message into the queue.
(2) \textit{Construct the Record Section of the Message:}
Constructing the record section of a message involves (i) checking if the queue needs
resizing, (ii) generating and inserting a rejected message record if needed,
(iii) refreshing older live records before they are evicted,
(iv) inserting the record from the key value store layer, and
(v) filling unused space in the 
record section with old live records in need of
a refresh.
(3) \textit{Send the Message:} The client next sends the message
to the server.  If the server rejects the message because it has an
old sequence number, then the server returns the newer messages to
prove that the rejected message was in fact old.  The client then
processes all of the new messages that were returned by the server and
will generate a rejected message record to communicate the fact that
it sent a message that was rejected.  If the server accepts the
message, then the client's local state is updated using the contents
of the newly created message.  If sending the message fails due to
network issues then the message passing layer has to defer its
determination of whether other clients received the message and the
transactional key-value store layer is informed that a network failure
occurred.

\myparagraph{Information Leakage}
A reader may note that the pattern of \putmsg and \getmsg requests
can leak access pattern information.  This issue
can be addressed in several different ways.  We modified
the update procedure to always follow a \getmsg call with a \putmsg call (simply sending a message that refreshes entries if there is no request to send).
Nevertheless, \TOOL does not prevent leaks
via timing channels.  For some settings, it is feasible to
configure \TOOL to not leak information by sending data on a
fixed schedule.\footnote{
We have observed that many smart home devices frequently send messages
to the cloud even when idle: the Nest thermostat sends a packet every
5 seconds, the LiFX light bulb every 7 seconds, and the D-Link smart
plug every 1.5 seconds.}

\myparagraph{Strengthening Consistency Guarantees}\label{sec:consistency}
Although we believe that fork consistency is sufficient for smart home systems,  
\TOOL supports extensions to counter forking attacks and achieve strong consistency~\cite{technicalreport}.

\mysubsection{Transactional Key-Value Store}\label{sec:kvstore}
\TOOL's transactional key-value store is built on top of the
message passing layer.
This layer
(1) arbitrates/commits transactions, and
(2) updates/reads key-value pairs.
%The application code runs on top of these two layers in each client. On smart home devices, this code is the device controller code.  On smartphones, this is the actual app code. 

\mycomment{
\begin{figure}[!htb]
\vspace{-1.1em}
\includegraphics[scale=0.35]{figures/Arbitrator.pdf}
\vspace{-1.5em}
\caption{\label{fig:conflict}Example Arbitration Scenario}
\vspace{-0.5em}
\end{figure}
}

\myparagraph{Arbitrating/Committing Transactions}
Intermittent home Internet connectivity complicates committing transactions.  There is the potential for concurrent local updates and remote updates to conflict.  In the case of an Internet outage, the cloud server would not even be aware of local updates. %Figure~\ref{fig:conflict} shows a scenario in which the home Internet connection has failed and there are two smartphones trying to control the thermostat.   A remote smartphone attempts to change the thermostat mode from 
For example, a remote smartphone attempts to change the thermostat mode from
HEAT to OFF with a transaction.  At the same time, a local smartphone tries to change the mode from HEAT to COOL with a transaction. These two transactions conflict and only one transaction can commit and thus we need an \emph{arbitrator} to decide which one commits.  
To allow local control during an Internet outage, the arbitrator of this transaction must be local to the thermostat and the obvious choice is the thermostat itself.

\myparagraph{Updating/Reading Key-Value Pairs}
\TOOL updates key-value pairs through a \code{Put} function. 
%(see Figure~\ref{fig:modeset}).
These updates are stored locally until the transaction is committed.
\TOOL supports a relaxed transactional model for reads.
In many cases it is not
important that a transaction reads the absolutely latest value from a
sensor. 

\mycomment{
\TOOL provides two get functions for this purpose:
(1) \code{GetCommittedAtomic:} This accessor function ensures
serializability (\ie isolation).
%: it is implemented by
%incorporating a guard into each transaction: the guard consists of a
%set of key-value pairs that must be present for the transaction to
%commit.\footnote{
%For example, if a call to \code{GetCommittedAtomic(Mode)} returned \code{HEAT}, \TOOL 
%would add the key-value pair $\tuple{\code{Mode}, \code{HEAT}}$ to the guard set \code{G}.}
%The enclosing transaction would then abort if this key-value pair was not present. 
%To commit a transaction, the arbitrator validates the guard:
%if all key-value pairs are present, the transaction is committed.
%Otherwise, the arbitrator aborts the transaction:
%applications receive a \javacode{TransactionStatus} object
%that allows the application to take the appropriate action 
%(see Figure~\ref{fig:modeset}).
(2) \code{GetCommitted:} 
This function allows accesses to violate transaction
serializability without causing a transaction to abort.  This can be
useful to read data values for which the application only needs
approximately current information.
}

\mycomment{
In many cases, it is desirable to allow interactive updating of a
device's state without waiting for the device to contact the cloud.
Even if the network connectivity is lost, such transactions are unlikely 
to actually conflict.  \TOOL supports a speculative 
get operation that reads values from pending transactions.
}


==> kvstore.tex <==
\mysection{Transactional Key-Value Store}\label{sec:kvstore}

We next present the transactional key-value store.
\TOOL's transactional key-value store is built on top of its message passing layer.  It relies on the message passing layer to ensure that the transactional key-value store layer receives a consistent set of messages from the server.

\mysubsection{Transaction Operations}

We next present the set of operations the transactional key-value store supports:
\squishlist
\item {\bf Assigning an Arbitrator:}
Before a key can be used it must be created and
assigned an arbitrator using a method which creates a new key record. If the key already exists or if the creation
fails the client will be notified.  The arbitrator of each key
$\mathsf{k}$ is stored with a new key record, which records the device 
that arbitrates the key $\mathsf{k}$.

\item {\bf Updating Key-Value Pairs:}
Transactions update key-value pairs by using the \code{Put} function.
These updates are stored locally until the transaction is committed.

\item {\bf Looking up Keys:}
A transaction can retrieve the values that are paired with keys using
the \code{GetCommittedAtomic} or the \code{GetCommitted} functions.
Recall that accesses using the \code{GetCommittedAtomic} functions
ensure serializability and thus introduce guard conditions that must
be checked when committing the transaction.

\item{\bf Commiting Transactions:}
To commit a transaction, the client creates a transaction record.
A transaction record is a tuple\mycomment{,
$\tuple{\sserver, \stlocal, \id, \KV{}, \MYG{}}$} that is comprised of
the set $\KV{}$ of key-value pairs \mycomment{---a key-value pair is
$\tuple{k,v}$---}to be updated, the guard condition $\MYG{}$ that
consists of the set of key-value pairs to be validated before
committing the transaction, and the sequence number $\sserver$ of
the message that first contained the transaction record.  The
combination of the machine ID $\id$ that created the transaction
and the client's local transaction sequence number $\stlocal$ is used
to uniquely specify the transaction.

The client then attempts to send the record to the server or in the event of
a network failure tries to send the record to the arbitrator.
\TOOL returns a future that the client can use to check 
whether a transaction committed.

Once a transaction record has been created, the client code
attempts to send it to the server.  Recall that multiple clients might
make \putmsg requests to the server simultaneously. This can cause
the \putmsg requests to fail.  If this occurs, the client simply
retries sending the same transaction record.  Note that this merely
reattempts sending the record and does not retry the underlying
transaction.  Furthermore, there may be more records that need to be
sent than a message can fit, and thus clients may need to send
multiple messages to enqueue all pending record data into the queue.

In the event of a network failure, the client falls back to local
communication and sends transactions directly to the arbitrator if local
communication is possible.
\squishend

\mysubsection{Arbitrating Transactions}

As stated previously each key is arbitrated by a specific device to
support committing transactions even when server connectivity is lost.
An arbitrator commits a transaction by evaluating the guard condition
$\MYG{}$ of that transaction to verify that that transaction is
serializable. This allows transactions to be predicated on specific
key-value pairs from the current committed set of key-value pairs at
the time when the transaction was created. When a transaction is
arbitrated, if the transaction is not serializable, \ie at least one
of the $\tuple{k,v} \in \MYG{}$ is not contained in the current set of
committed key-value pairs, then all key-value updates in $\KV{}$ are
ignored and the transaction is aborted. Otherwise, the updates are
performed and the transaction is committed.

When a transaction arbitrator decides to commit a transaction, it
creates a commit record
\mycomment{$\tuple{\sserver, \arbLocalId, \tLocalId,\\ \KV{}}$} to record the
updates to key-value pairs.  A commit record contains the set $\KV{}$
of updated key-value pairs.  The record also contains the sequence
number $\sserver$ of the message that first contained the commit
record, the arbitrator's machine ID $\idarblocal$ and local
arbitration sequence number $\sarblocal$, and the pair of the machine ID
$\idtlocal$ and the local transaction sequence number $\stlocal$,
which together uniquely specifies the original transaction.  A $\commit$
record keeps track of the updated key-value pairs.  Thus, a $\commit$
record is live until every key-value pair in the commit record is overwritten by newer commits.

If an arbitrator decides to abort a transaction, it creates an abort
record \mycomment{$\tuple{\sserver,\arbLocalId, \tLocalId}$} to inform the client
that created the transaction that the transaction has not been
accepted.  The abort record contains the sequence number $\sserver$ of
the message that first contained the abort record, the arbitrator's
machine ID $\idarblocal$ and local arbitration sequence number
$\sarblocal$, and the machine ID $\idtlocal$ and the local transaction
sequence number $\stlocal$, which uniquely specifies the original
transaction.  Since abort records are used by the server to notify
the client that generated a transaction that the transaction aborted,
an abort record is live until the client that generated the
transaction has confirmed the receipt of the abort record by inserting
a message with a sequence number that is larger than the abort's
sequence number.

After arbitration, commits and aborts are sent to the server
so that clients may see them.  In the event of a network failure,
clients can request commits and aborts be passed locally.

Transaction records are processed by arbitrators in order of
$\sserver$.  Thus, a commit or abort for a transaction with $\sserver$
implies that all transactions with the same arbitrator as that
transaction (but with a smaller $\sserver$) have been arbitrated and
that the transaction record is no longer live.

\mysubsection{Processing Commit and Abort Records}

Abort records do not require any processing since their purpose is (1)
to mark a transaction record dead and (2) to allow clients to be
notified of aborted transactions.  Commit records are stored in a
temporary buffer and processed after all commit records from the new
messages have been extracted since they may be received out of order
and thus need to be sorted before they can be processed.

Clients can obtain the latest key-value pairs by requesting and
processing new messages from the server.  During the update process,
all pending commits, aborts, and transactions that have not been
enqueued to the server, or passed locally in the case of transactions,
are enqueued using the same method described above. If the server is
not reachable, then key-value pairs can be updated using local
communication by requesting all new commits and aborts directly from
the key's arbitrator.


\mysubsection{Handling Network Failures}

As a result of an ill-timed network failure during an attempt by a
client to enqueue a message that contains a transaction record,
a client could have successfully inserted a transaction record into
the queue but not received a response from the server.  If local
communication is not possible then the client will try to enqueue the
same transaction at a later time.  If a transaction
happens to be sent twice, the arbitrator will detect this by
comparing the transaction records' $\tLocalId$ tuple and ignore
the second copy.  If local communication occurs then there is a chance
that an arbitrator will see the same transaction record twice, once
from the server and once directly from the client.  As in the previous
case, the arbitrator will detect the duplication and ignore the second
copy.






\mycomment{
\mysubsection{Implementation}

Our implementation includes extra functionality including: (1) support
for transactions and key-value pairs of any
size, (2) commit compression that combines multiple commits to save
space, and (3) a presumed commit optimization.  This functionality is
described in Appendix~\ref{sec:opt}.% of the technical report~\cite{technicalreport}.
}








==> makefile <==
LATEX := pdflatex -halt-on-error

.SUFFIXES : .tex .bbl .aux .eps .ps .dot .pdf

.tex.bbl:
	bibtex $*

.tex.aux:
	latex $*

%.eps: %.ps
	ps2epsi $< $@

%.ps: %.dot
	dot -Tps $< -o $@

%.pdf: %.dot
	dot -Tpdf $< -o $@

%.png: %.dot
	dot -Tpng $< -o $@

%.aux: %.tex
	$(LATEX) $<

# latex the paper (default)
new:	biblinks newpaper

# latex + bibtex the paper
bib:	bibpaper newpaper


biblinks: figures
	$(LATEX) paper.tex
	bibtex paper.aux
	$(LATEX) paper.tex

newpaper: figures biblinks
	$(LATEX) paper.tex

bibpaper: paper.aux paper.bbl
	latex paper.tex

spell:
	@for i in *.tex; \
	do if [ $$i != "paper.tex" ]; then aspell -c $$i -p ./spell.lst; fi;\
	done


total:
	pdflatex paper.tex
	bibtex paper.aux
	pdflatex paper.tex
	pdflatex paper.tex
	@echo ================================================================
	pdflatex paper.tex | grep -E 'arning|erfull'
	@echo ================================================================


figures: $(FIGURES)



clean:
	rm -f *.dvi *.log *.aux *.blg *.bbl *~
	rm -f paper.ps paper.pdf 


==> opt.tex <==
\mysection{Implementation}\label{sec:opt}

Our implementation has extra functionality and
optimizations including
support for transactions of any size.

\myparagraph{Arbitrary Sized Key-Value Pairs and Transactions}
Our implementation supports key-value pairs of any size.  Our implementation does not require
individual commits and transactions fit in a single fixed-size message.
Our
implementation instead allows transactions and commits to be broken into 
parts.  Key-value data is broken into parts and span as
many records as needed.  Transactions 
and commits are pieced together from their parts to recover the key-value
data for commit and transaction processing.

\myparagraph{Transaction Speculation}

Recall that many IoT devices are only intermittently online to save power.  We
also expect that the cloud server would typically be reachable and
thus local communication would infrequently occur.  Thus our implementation supports
transaction speculation---an optimization that allows clients to
obtain key-value pairs from transactions before the transactions are
actually committed by the arbitrator.  This optimizes for the common
case and allow clients to provide a more interactive experience.

This optimization is implemented by examining the set of committed
key-value pairs and the set of pending-arbitration transactions to determine the
set of transaction commit decisions that the arbitrator will make assuming
that there are no locally communicated transactions.  Clients may 
use the speculative values as guard conditions for future
transactions.

\myparagraph{Commit Compression}
During arbitration many transactions that operate on the same
key-value pairs may be arbitrated together.
For example, this can happen when an arbitrator is offline for a period of
time and then pulls messages from the server. This may
cause some commits to contain key-value pairs that have been
overwritten by a newer commit processed in the same batch.
To avoid sending commit information that will immediately be
overwritten our implementation compresses several commits
into one or more larger commits.  Multiple updates to the same key-value
pair from multiple commits will be compressed to only a single
update with that single update being the update from the most recent
commit.  This new commit will be at most as large as the sum of the
sizes of commits it compresses but could be significantly smaller if
many commits updated the same keys. When a commit
becomes very large or a part of the commit has been sent, it will
no longer be compressed.

We also have a presumed commit optimization---if a
transaction with a later identifier is processed, early committed
transactions are presumed to have committed and the commit records can
be elided.  Thus, it is important to maintain constraints
on the relative ordering of commits and aborts---aborts must appear
at least as early as they did in the original order to ensure that they are not presumed to have committed.  If an abort
appears in the middle of a sequence of commits that is compressed, it
must be sent before the commits.

%Our implementation includes extra functionality including: (1) support
%for transactions and key-value pairs of any
%size, (2) commit compression that combines multiple commits to save
%space, and (3) a presumed commit optimization.  This functionality is
%described in Appendix~\ref{sec:opt}.% of the technical report~\cite{technicalreport}.




==> overview.tex <==
\mysection{Overview}\label{sec:overview}

\begin{figure}[!htb]
\vspace{-.5em}
\begin{center}
\includegraphics[scale=0.43]{figures/BlockChain}
\end{center}
\vspace{-1.4em}
\caption{Message Chain\label{fig:messagechain}}
\vspace{-1.em}
\end{figure}

\TOOL uses a message chain to provide secure, totally ordered
communications between clients.  Since the server is not trusted, the
clients must be able to locally verify the integrity of the message
chain.  Therefore, each message in the chain has a fixed size and
contains a unique sequence number, a keyed-hash message authentication
code (HMAC) of the previous message in the chain, and a set of
records.  Finally, each message contains an HMAC of itself.  This
ensures that the message cannot be modified.  The HMACs are generated
using a key known only to the clients to ensure that the server cannot forge
messages.  When a message is transported between clients, it is always
encrypted using the transport key.  Together, this ensures that the
server cannot know the contents of messages nor can it modify them.

\paragraph{Message Truncation and Refreshing Records}
A simple message chain would eventually consume all memory on the
devices and server.  Thus, \TOOL is designed such that the last $n$
messages in the chain have enough information to reconstruct the state
of the key value store.  This enable \TOOL to truncate the message
chain.  An important secondary benefit of truncating the message chain
is that the amount of work that a client that goes to sleep and then
wakes after a long period of time must perform is bounded by $n$.

Records in the key-value store can potentially be long-lived.  Thus a
consequence of our design choice is that such records must be
reinserted into the message chain (or refreshed) before they are
truncated.


==> proof.tex <==
\mysection{Security of Message Passing}\label{sec:proof}

A second security concern is ensuring that the server cannot corrupt
communications between clients.  HMACs ensure the integrity of
individual messages, but do not prevent the server from sending old
message, accepting multiple messages with the same sequence number,
etc.  We thus prove a theorem that if two devices receive the same
message, then all previous messages they have received are consistent.


\mycomment{\begin{theorem}
Suppose that there is a transitive closure set $\mathsf{\mathscr{S}}$
of clients, at sequence number $\mathsf{n}$. Then there is some
total sequence $\mathsf{T}$ of length $\mathsf{n}$ such that every
client~$\mathsf{C}$ in $\mathsf{\mathscr{S}}$ sees a partial sequence
$\mathsf{P_C}$ consistent with $\mathsf{T}$.
\end{theorem}

\begin{proof}
See Appendix~\ref{sec:proof}.
\end{proof}}


In this Section, we present the guarantees provided by the message
passing layer.  We start by presenting several definitions and then prove several properties.  

\begin{defn}[Equality]
Two messages $\mathsf{t}$ and $\mathsf{u}$ are equal if their
$\mathsf{s}$ and $\mathsf{Dat_t}$ are equal.
\end{defn}

\begin{defn}[Parent]
A parent of a message $\mathsf{t}$ is the message $\mathsf{p_t}$, 
unique by the correctness of HMACs in $\mathsf{Dat_t}$, such that 
$\mathsf{hmac_p(t) = hmac_c(p_t)}$.
\end{defn}

\begin{defn}[Chain]
A chain of messages with length $\mathsf{n \ge 1}$ is a message
sequence $\mathsf{R = (r_s, r_{s+1}, ..., r_{s+n-1})}$ such that for
every sequence number $\mathsf{s < k \le s+n-1}$, $\mathsf{r_k}$ has
sequence number $\mathsf{k}$ and its parent is $\mathsf{r_{k-1}}$.
\end{defn}

\begin{defn}[Partial sequence]
A partial sequence $\mathsf{P}$ is a sequence of messages, no two with
the same sequence number, that can be divided into disjoint chains.
\end{defn}

\begin{defn}[Total sequence]
A total sequence $\mathsf{T =}$ $\mathsf{(t_1, t_2, ..., t_n)}$ with
length $\mathsf{n}$ is a chain of messages that starts at $\mathsf{s =
  1}$.
\end{defn}

\begin{defn}[Path]
The path of a message $\mathsf{t}$ is the total sequence whose last
message is $\mathsf{t}$. The uniqueness of a path follows from the
uniqueness of a parent.
\end{defn}

\begin{defn}[Consistency]
A partial sequence $\mathsf{P}$ is consistent with a total sequence
$\mathsf{T}$ of length $\mathsf{n}$ if for every message $\mathsf{p
  \in P}$ with sequence number $\mathsf{s_p \leq n}$, $\mathsf{t_{s_p} = p}$. This
implies that $\mathsf{\{p \in P | s_p \le n\}}$ is a partial sequence
of $\mathsf{T}$.
\end{defn}

\begin{defn}[Transitive closure]
The transitive closure set at sequence number $\mathsf{s_n}$ is a set
$\mathsf{\mathscr{S}}$ of clients comprising a connected component of
an undirected graph, where two clients are connected by an edge if
they both received the same message $\mathsf{t}$ with sequence number
$\mathsf{s_t > s_n}$.
\end{defn}


\begin{prop}
\label{prop:parentmessage}
Every client~$\mathsf{J}$ who sends a message $\mathsf{t}$ has parent
$\mathsf{p_t}$ as its latest stored message and $\mathsf{s_t =
  s_{p_t} + 1}$.
\end{prop}
\begin{proof} True by construction, because client~$J$ sets 
$\mathsf{hmac_p(t) = hmac_c(p_t)}$ and $\mathsf{s_t = }$
  $\mathsf{s_{p_t + 1}}$ when a message is sent.
\end{proof}

\begin{prop} 
\label{prop:rejectedmessage}
If a rejected message record is added to the queue at
sequence number $\mathsf{s}$, the record will remain in the queue
until every client has seen it.
\end{prop}
\begin{proof}
Every record $\de{}$ remains in the queue until it
reaches the tail, and is refreshed by the next sender $\mathsf{J}$ at
that time until every client
has sent a message with a sequence number greater than
$\mathsf{s}$. Because every client who sends a message with
sequence number $\mathsf{s'}$ has a copy of the entire queue at
$\mathsf{s' - 1}$, this client will have seen the message at
$\mathsf{s}$.
\end{proof}

\begin{figure}[!htb]
\resizebox{.5\textwidth}{!}{
  \centering
      \xymatrix{ & & L \\
\dots \ar[r] & q \ar[dr]_{J} \ar[r]^{K} & l_1 \ar[r] & l_2 \ar[r] & \dots \ar[r] & m \ar[r] & \dots \ar[r] & l_n = u \\
& & r_1 \ar[r] & r_2 \ar[r] & \dots \ar[r] & r_m = t \\
& & R
\save "2,3"."2,8"*+\frm{^\}}
\save "3,3"."3,6"*+\frm{_\}}
\restore
\restore
      }
      }
\caption{By \textbf{Lemma~\ref{lem:twomessages}}, receiving both $t$
  and $u$ here is impossible.\label{fig:fork}}
\end{figure}


\begin{lem}
\label{lem:twomessages}
If two messages, $\mathsf{t}$ and $\mathsf{u}$, such that $\mathsf{s_t \le s_u}$
are received by a client~$\mathsf{C}$ without any clients reporting errors,
then $\mathsf{t}$ is in the path of $\mathsf{u}$.
\end{lem}
\begin{proof}
Assume that there are some pairs of messages $\mathsf{(t,u)}$ that
violate this lemma for some client~$\mathsf{C}$.  Take a specific pair
$\mathsf{(t,u)}$ and client~$\mathsf{C}$ such that $\mathsf{s_u}$ is
minimized, and $\mathsf{s_t}$ is maximized for this choice of
$\mathsf{s_u}$. We will show that client~$\mathsf{C}$ cannot receive both
$\mathsf{t}$ and $\mathsf{u}$ without some client throwing an error.

Clearly client~$\mathsf{C}$ will throw an error if $\mathsf{s_t = s_u}$. So
$\mathsf{s_t < s_u}$. Additionally, if client~$\mathsf{C}$ receives
$\mathsf{u}$ before $\mathsf{t}$, this will cause it to throw an
error, so $\mathsf{t}$ must be received before $\mathsf{u}$. We will prove
that an error occurs upon receipt of $\mathsf{u}$.

Let $\mathsf{r_1}$ be the earliest member of the path of $\mathsf{t}$
that is not in the path of $\mathsf{u}$, and let $\mathsf{q}$ be its
parent. Message $\mathsf{q}$, the last common ancestor of $\mathsf{t}$
and $\mathsf{u}$, must exist, since all clients and the server were
initialized with the same state. Let $\mathsf{l_1}$ be the successor
of $\mathsf{q}$ that is in the path of $\mathsf{u}$; we know
$\mathsf{l_1 \neq r_1}$. Let $\mathsf{R = (r_1, r_2, \dots, r_{|R|} =
  t)}$ be the distinct portion of the path of $\mathsf{t}$, and
similarly let $\mathsf{L}$ be the distinct portion of the path of
$\mathsf{u}$.

Let $\mathsf{J}$ be the client who sent $\mathsf{r_1}$; that is, such
that $\mathsf{{id_{self}}_J = GetMacID(r_1)}$, and $\mathsf{K}$ be the
client who sent $\mathsf{l_1}$. Because no client can send two
messages with the same sequence number, and $\mathsf{s_{r_1} = s_{l_1}
  = s_q + 1}$, $\mathsf{J \neq K}$.

We next prove the two propositions that we will use to complete this
proof.

\begin{prop} 
\label{prop:bothmessages}
No client sends both a message in $\mathsf{(r_2,...,t)}$ and a message
in $\mathsf{(l_2,...,u)}$.
\end{prop}

\begin{proof}
To send a message $\mathsf{p}$ that is the parent of some other
message, one must have received the parent of $\mathsf{p}$. Since
$\mathsf{u}$ is the message with smallest sequence number received by
any client that violates Lemma~\ref{lem:twomessages}, no client can
receive both a message in $\mathsf{r}$ and a message in $\mathsf{l}$.
\end{proof}

\begin{prop} 
\label{prop:seqnumb}
Client~$\mathsf{C}$ does not receive any message with a sequence number
strictly between $\mathsf{s_t}$ and $\mathsf{s_u}$.
\end{prop}

\begin{proof}
If there were such a message with sequence number smaller than
$\mathsf{s_u}$, it would contradict the assumption that $\mathsf{u}$
is the message with the least sequence number that violates
Lemma~\ref{lem:twomessages}.
\end{proof}

We continue the proof of Lemma~\ref{lem:twomessages}.  There are two cases:
\begin{itemize}
\item Case 1: Client~$\mathsf{J}$ did not send a message in
  $\mathsf{L}$. Define $\mathsf{s_{t_J}}$ to be the greatest sequence
  number of the messages that client $\mathsf{J}$ sent in the path of
  message $\mathsf{t}$.  Define $\mathsf{s_{q_J}}$ and
  $\mathsf{s_{u_J}}$ similarly.  We then have $\mathsf{s_{t_J} >
    s_{q_J} = s_{u_J}}$.
\begin{itemize}
\item Case 1.1: Client~$\mathsf{C}$ never calls $\code{ValidateLastMessages()}$
  between receiving $\mathsf{t}$ and receiving $\mathsf{u}$; by
  Proposition~\ref{prop:seqnumb} this can only happen if $\mathsf{s_t
    = s_u - 1}$. Since $\mathsf{t}$ is not the parent of $\mathsf{u}$,
  $\mathsf{hmac_p(u) \neq hmac_c(t)}$, causing client~$\mathsf{C}$ to throw
  an error.
\item Case 1.2: Case 1.1 does not occur; therefore, client~$\mathsf{C}$ calls
  $\code{ValidateLastMessages()}$ at some point between receiving
  $\mathsf{t}$ and $\mathsf{u}$.  The latest sequence number of
  client~$\mathsf{J}$ decreases during this time, which means client~$\mathsf{C}$
  throws an error in the $\code{ValidateLastMessages()}$ function.
\end{itemize}
\item Case 2: Client~$\mathsf{J}$ sent at least one message in
  $\mathsf{L}$. Call the first one $\mathsf{m}$. We know that
  $\mathsf{s_m > s_{r_1}}$, since $\mathsf{J \neq K}$ and $\mathsf{m
  \neq l_1}$.  Since the current sequence number for $\mathsf{J}$ can
  only increase, client~$\mathsf{J}$ must send the message
  $\mathsf{r_1}$ before the message $\mathsf{m}$.  Let $\mathsf{X =
    (r_1 = x_1, \dots, x_n)}$ be the list of messages client~$\mathsf{J}$
  sends starting with $\mathsf{r_1}$ and ending immediately before $m$; clearly
  these all have sequence number $\mathsf{\geq s_q + 1}$.
\begin{itemize}
\item Case 2.1: Some message in $\mathsf{X}$ was accepted by the
  server. Therefore, before sending $\mathsf{m}$, client~$\mathsf{J}$'s value
  in $\code{lastmessage}$ for its own latest sequence number would be
  greater than $\mathsf{s_{q_J}}$. If there is a sequence of messages
  with contiguous sequence numbers that client~$\mathsf{J}$ receives
  between $\mathsf{r_1}$ and $\mathsf{m}$ (switching from the
  $\mathsf{R}$ chain to the $\mathsf{L}$ chain), client~$\mathsf{J}$
  throws an error for a similar reason as Case 1.1. Otherwise, when
  preparing to send $\mathsf{m}$, client~$\mathsf{J}$ would have
  received an update of its own latest sequence number as at most
  $\mathsf{s_{q_J}}$. Client~$\mathsf{J}$ throws an error before
  sending $\mathsf{p}$, because its own latest sequence number
  decreases.

\item Case 2.2: All messages in $\mathsf{X}$ were rejected by the
  server, making $\mathsf{m}$ the first message of client~$\mathsf{J}$
  that is accepted after $\mathsf{r_1}$.

We will prove that client~$\mathsf{C}$ sees $\mathsf{r_1}$ by
contradiction. Assume not. Then $\mathsf{(r_2, ..., t)}$ must have at
least $\currqsize_C \geq 2$ messages for $\mathsf{r_1}$ to fall off
the end of the queue (note that by Proposition~\ref{prop:seqnumb}
client~$\mathsf{C}$ cannot receive the next message after
$t$). Consider the sender of $\mathsf{r_3}$ and call it $\mathsf{H}$.
$\mathsf{H \neq J}$ by Proposition~\ref{prop:bothmessages} and the
existence of $\mathsf{m}$.  Since $\mathsf{H \neq J}$, then by
Proposition~\ref{prop:bothmessages} it could not also have sent a
message in $\mathsf{(l_2,..., u)}$. Therefore, $\mathsf{s_{u_H} < s_q
  + 2 = s_{t_H}}$, so upon receipt of $\mathsf{u}$, client~$\mathsf{C}$ will
throw an error by the decrease in a last sequence number similar to
Case 1, a contradiction.

Now that we know that client~$\mathsf{C}$ must receive
message~$\mathsf{r_1}$, note that client~$\mathsf{C}$ receives
$\mathsf{u}$ immediately after $\mathsf{t}$ by
Proposition~\ref{prop:seqnumb}. Therefore, client~$\mathsf{C}$ could not have
seen a message after $\mathsf{t}$ with sequence number less than
$\mathsf{s_m}$. In the $\code{AttemptSendRecord()}$ function,
client~$\mathsf{J}$ adds a rejected message record that contains sequence
number $\mathsf{s}$ and its machine ID to record the rejected
messages.  Hence, for every $\mathsf{i}$, $\mathsf{1 \leq i < |X|}$,
the rejected message $\mathsf{x_i}$ from client~$\mathsf{J}$ will be
recorded. Since all the rejected message records that store the rejected
messages will also be seen when $\mathsf{u}$ is received, and
client~$\mathsf{C}$ sees $\mathsf{r_1}$, ${r_1}$ will be recorded as a
rejected message.  When client~$\mathsf{C}$ receives $\mathsf{u}$, it will
throw an error due to previously having received a message that was
marked as rejected.
\end{itemize}
\end{itemize}
\end{proof}

\begin{lem} 
\label{lem:pathmessages}
If there are two messages $\mathsf{t}$ and $\mathsf{u}$, with
$\mathsf{s_t \leq s_u}$, such that $\mathsf{t}$ is in the path of
$\mathsf{u}$, then for any message $\mathsf{p}$ with $\mathsf{s_p \leq
  s_t}$, iff $\mathsf{p}$ is in the path of $\mathsf{t}$, it is in the
path of $\mathsf{u}$.
\end{lem}

\begin{proof}
If $\mathsf{s_t = s_u}$ or $\mathsf{s_p = s_t}$, then we are done,
because the two relevant messages are the same. If they are different
messages, then:
\begin{itemize}
\item Reverse direction: The definition of $\mathsf{t}$ being in the
  path of $\mathsf{u}$ is the existence of a message sequence
  $\mathsf{(\dots, t, \dots, u)}$ such that each message except
  $\mathsf{u}$ is the parent of the succeeding message.  The path of
  $\mathsf{u}$ must contain some message with sequence number
  $\mathsf{s_p}$; because $\mathsf{p}$ is in the path of $\mathsf{u}$,
  this message is $\mathsf{p}$ itself. The path of $\mathsf{t}$ is
  then the prefix of this path ending at $\mathsf{t}$, which clearly
  contains $\mathsf{p}$.

\item Forward direction: The path of $\mathsf{t}$ is a substring of
  the path of $\mathsf{u}$, so if the path of $\mathsf{t}$ contains
  $\mathsf{p}$, so does the path of $\mathsf{u}$.
\end{itemize}
\end{proof}

\begin{theorem}
Suppose that there is a transitive closure set $\mathsf{\mathscr{S}}$
of clients, at sequence number $\mathsf{n}$. Then there is some
total sequence $\mathsf{T}$ of length $\mathsf{n}$ such that every
client~$\mathsf{C}$ in $\mathsf{\mathscr{S}}$ sees a partial sequence
$\mathsf{P_C}$ consistent with $\mathsf{T}$.
\end{theorem}

\begin{proof}
The definition of consistency of $\mathsf{P_C}$ with $\mathsf{T}$ is
that every message $\mathsf{p \in P_C}$ with sequence number
$\mathsf{s_p \le n}$ is equal to the message with that sequence number in
$\mathsf{T}$. Let $\mathsf{C_1}$ be some client in the transitive
closure set, with partial sequence $\mathsf{P_{C_1}}$, and let
$\mathsf{u}$ be some message with $\mathsf{s_u > n}$ that
$\mathsf{C_1}$ shares with another client. Then let $\mathsf{T}$ be
the portion of the path of $\mathsf{u}$ ending at sequence number
$\mathsf{n}$ and $\mathsf{t}$ be the message at that sequence
number. Clearly, by Lemma~\ref{lem:twomessages}, $\mathsf{P_{C_1}}$ is
consistent with $\mathsf{T}$. We will show that, for every other
client $\mathsf{D}$ with partial sequence $\mathsf{P_D}$,
$\mathsf{P_D}$ has some message whose path includes
$\mathsf{t}$. Because $\mathsf{D}$ is in the transitive closure, there
is a sequence of clients $\mathsf{\mathscr{C} = (C_1, C_2, ..., D)}$
from $\mathsf{C_1}$ to $\mathsf{D}$, where each shares an edge with
the next.  We prove by induction that $\mathsf{P_D}$ has a message
whose path includes $\mathsf{t}$.
\begin{itemize}
\item Base case: $\mathsf{P_{C_1}}$ includes $\mathsf{u}$, whose path
  includes $\mathsf{t}$.

\item Inductive step: Each client in $\mathsf{\mathscr{C}}$ has a
  partial sequence with a message that includes $\mathsf{t}$ if the
  previous client does. Suppose $\mathsf{P_{C_k}}$ has a message
  $\mathsf{w}$ with a path that includes $\mathsf{t}$, and shares
  message $\mathsf{x}$ with $\mathsf{P_{C_{k+1}}}$ such that
  $\mathsf{s_x > n}$. By Lemma~\ref{lem:twomessages}, $\mathsf{w}$
  or $\mathsf{x}$, whichever has the least sequence number, is in the
  path of the other, and therefore by Lemma~\ref{lem:pathmessages},
  $\mathsf{t}$ is in the path of $\mathsf{x}$.

\item Let $\mathsf{z}$ be the message of $\mathsf{D}$ whose path
  includes $\mathsf{t}$.  By Lemma~\ref{lem:twomessages}, every
  message in $\mathsf{P_D}$ with sequence number smaller than
  $\mathsf{s_w}$ is in the path of $\mathsf{z}$. Since $\mathsf{t}$ is
  in the path of $\mathsf{z}$, every message in $\mathsf{P_D}$ with
  smaller sequence number than $\mathsf{s_t = n}$ is in
  $\mathsf{T}$.  Therefore, $\mathsf{P_D}$ is consistent with
  $\mathsf{T}$.
\end{itemize}
\end{proof}


==> pseudocode.tex <==
\newpage
\mysection{Key Value Store Pseudocode}\label{sec:pseudocode}
\begin{figure}[!htb]
  \footnotesize
  \begin{algorithmic}[1]
    \Function{ValidateandUpdate}{Messages[] $\newmsgs$}
      \If{$|\newmsgs| = 0$}
        \State{\Return{}}
      \EndIf
      \State{$\code{ResetQueueSizeCounter}()$}
      \State{Check that first message has a sequence number that is $\geq \seqnum$.}
      \ForAll{$\fullmsg$ in $\newmsgs$}
        \State{Decrypt $\encpayload$ to obtain $\payload$.}
        \State{Validate that $\seqnume = \seqnum$.}
        \State{$\code{Validate}(\payload)$.}
        \State{$\code{IncrementQueueSizeCounter}()$}
      \EndFor

      \If{Gap exists between $\localqueue$ and $\newmsgs$}
      \State{$\code{ValidateQueueSizeCorrect}(|\newmsgs|)$}
      \State{$\code{ValidateLastMessages}()$}
      \EndIf
    \If{we sent a message that is still unresolved}
    \State{Create reject message entry for message}
    \EndIf
    \State{Update $\qsize$ using $\currqsize$ and resize $\localqueue$.}
      \State{$\code{UpdateLastMessages}()$}
      \State{Add decrypted $\newmsgs$ to $\localqueue$.}
      \State{Update $\currseqnum$.}
      \State{$\code{processKVStore}()$}
    \EndFunction
  \end{algorithmic}
\caption{\label{fig:validateupdate}Validate and Update Procedure}
\end{figure}

% Individual Message Validation
\begin{figure}[!htb]
  \footnotesize
  \begin{algorithmic}[1]
    \Function{Validate}{$\payload$}
      \State{Validate $\hmacc=HMAC(\payload)$.}
      \State{Validate $\hmacp=HMAC(\payload_{p})$.}
      \State{$\code{processLastMsg}(\tuple{\id,\seqnum})$}
      \ForAll{$\de{}$ in $\DE{}$}
        \If{$\de{}$ is a $\lastmsg$}
          \State{$\code{processLastMsg}(\de{})$}
        \ElsIf{$\de{}$ is a $\queuestate$}
          \State{$\code{processQueueStatus}(\de{}, \seqnume)$}
        \ElsIf{$\de{}$ is $\rejmsg$}
          \State{$\code{processRejectedMsg}(\de{})$}
        \Else
          \State{$\code{processKVStoreRecord}(\de{})$}
        \EndIf
      \EndFor
    \EndFunction
  \end{algorithmic}
\caption{\label{fig:validatemsg}Validate Individual Message}
\end{figure}

% Record Handlers
\begin{figure}[!htb]
  \footnotesize
  \begin{algorithmic}[1]
    \Function{processLastMsg}{$\tuple{\id, \seqnum'}$}
      \If{$\localid=\id \wedge \seqnum'$ is marked as unresolved}
      \State{Mark $\seqnum'$ as accepted and no longer unresolved}
      \EndIf
      \State{lastmsg[$\id$]:=$\seqnum'$}
    \EndFunction

    \Function{processQueueStatus}{$\tuple{n}, \seqnume$}
      \State{$\currqsize:=n$}
      \State{$\code{SetQueueSizeCounter}(\seqnume, n)$}
    \EndFunction

    \Function{processRejectedMsg}{$\rme$}
      \State{Validate that $\forall \tuple{\seqnum, \payload} \in \localqueue, \mathsf{s_{low}} \leq \seqnume \leq \mathsf{s_{high}} \Rightarrow \id_{\mathsf{rme}} \neq \id$ }
    \EndFunction
  \end{algorithmic}
\caption{\label{fig:messagehandler}Record Handlers}
\end{figure}

\newpage
\begin{figure}[!htb]
  \footnotesize
  \begin{algorithmic}[1]
    \Function{UpdateLastMessages}{}
    \ForAll{$\id$ in machines}
    \If{lastmsg[$\id$] $\neq 0$}
    \State{committedlastmsg[$\id$] = lastmsg[$\id$]}
    \EndIf
    \EndFor
    \EndFunction\\
    \Function{ValidateLastMessages}{}
    \ForAll{$\id$ in machines}
    \State{Validate lastmsg[$\id$] $\neq 0$}
    \State{Validate lastmsg[$\id$] $\geq$ committedlastmsg[$\id$]}
    \EndFor
    \State{Validate lastmsg[$\localid$] = our last accepted message}
    \EndFunction
    \end{algorithmic}
\caption{Last Message Validation\label{fig:lastmessage}}
\end{figure}

%\begin{figure}[!htb]
\begin{figure}[!htb]
  \footnotesize
  \begin{algorithmic}[1]
    % \Function{ResetQueueSizeCounter}{$\seqnume, n$}
    \Function{ResetQueueSizeCounter}{}
      \State{$\mathsf{counterReset} := \true$}
    \EndFunction\\

    \Function{SetQueueSizeCounter}{$\seqnume, n$}
      \If{$\mathsf{counterReset}$}
        \State{$\mathsf{counterReset} := \false$}
        \State{$\mathsf{expectedSize} := min(\seqnume, n)$}
        \State{$\mathsf{currentMaxSize} := n$}
      \EndIf
    \EndFunction\\

    \Function{IncrementQueueSizeCounter}{}
      \If{$\mathsf{expectedSize} < \mathsf{currentMaxSize}$}
        \State{$\mathsf{expectedSize} := \mathsf{expectedSize} + 1$}
      \EndIf      
    \EndFunction\\

    \Function{ValidateQueueSizeCorrect}{$n$}
      \State{Validate that $n = \mathsf{expectedSize}$}
    \EndFunction
  \end{algorithmic}
\caption{\label{fig:expectedmsgs}Compute Expected Number of Messages}
\end{figure}

\newpage
\begin{figure}[!htb]
  \footnotesize
  \begin{algorithmic}[1]
    \Function{SendRecord}{$\de{}$}
    \If{there is a message whose status is unresolved}
    \If{$\neg \code{ResendPastMessage}()$}
    \State{\Return{Had Server Timeout}}
    \EndIf
    \EndIf
    \State{forceresize:=$\false$}
    \State{$\DE{}:=\emptyset$}
    \If{$\code{ResizeThresholdReached()} \vee$ forceresize}\label{resize}
    \State{Calculate new queue size and resize threshold.}
    \State{$\DE{}:=\{$ New Resize Queue Record$\}$}
    \EndIf
    \State{$\DE{}:=\DE{} \cup $Generate $\rejmsg$ record for rejected msg list.}
    \If{$\lnot \code{MandatoryRefresh}(\DE{}) \land$ Not Resizing}
    \State{forceresize := $\true$}
    \State{$\DE{} := \emptyset$}
    \State{\Goto{resize}}
    \EndIf
    \If{$\code{HasSpace}(\DE{}, \de{})$}
    \State{$\DE{} := \DE{} \cup \{\de{}\}$}
    \EndIf
    \State{$\DE{} := \DE{} \cup$ Live records in other old messages that fit.}
    \State{$p:=\mathsf{\tuple{\currseqnum, \localid, \hmacp, \DE{} }}$.}
    \State{Send to server using: $\putmsg(\mathsf{\tuple{\currseqnum, E(\tuple{p, HMAC(p)}) }})$\label{putmessage}}
    \If{Server accepted message}
    \State{$\code{ValidateandUpdate}$($\mathsf{\tuple{\currseqnum, E(\tuple{p, HMAC(p)}) }}$)}
    \State{\Return{$\de{} \in \DE{}$}}
    \ElsIf{Server rejected message}
    \State{Add $\seqnum$ to rejected message list.\label{createrejectedmessage}}
    \State{$\code{ValidateandUpdate}$(Messages returned by server)\label{processservermessage}}
    \State{\Return{$\false$}}
    \ElsIf{Server never responds after timeout\label{networkissuestart}}
    \State{Mark message status as unresolved}
    \State{\Return{Had Server Timeout}\label{networkissueend}}
    \EndIf
    \EndFunction\\
\end{algorithmic}
\caption{\label{fig:sendrecord}Method to Send Record}
\end{figure}

\begin{figure}[!htb]
\begin{algorithmic}
  \footnotesize
    \Function{ResendPastMessage}{} 
      \State{Resend previous $\msg$ using: $\putmsg(\mathsf{\tuple{\currseqnum, E(\tuple{p, HMAC(p)}) }})$}
      \If{Server accepted message}
        % \State{Unmark message resent message $\seqnum$ as unresolved message}
        \State{$\code{ValidateandUpdate}(\mathsf{\tuple{\currseqnum, E(\tuple{p, HMAC(p)}) }})$}
        \State{\Return{$\true$}}
      \ElsIf{Server rejected message}
        % \State{Unmark message resent message $\seqnum$ as unresolved message}
        \If{Resent $\msg$ not in response $\land$ no $\lastmsg$ with same $\seqnume$ and $\id$ as $\msg$}
          \State{Add resent $\msg$ to rejected message list}
        \EndIf
        \State{$\code{ValidateandUpdate}$(Messages returned by server)}
        \State{\Return{$\true$}}
      \ElsIf{Server never responds after timeout}
        \State{\Return{Had Server Timeout}}
      \EndIf
    \EndFunction\\

    \Function{MandatoryRefresh}{$\DE{return}$}
    \If{oldest slot is unused}
    \State{\Return $\true$}
    \EndIf
    \State{Find the oldest $\tuple{s, \payload}$ in $\localqueue$}
    \ForAll{$e \in \DE{}$ that are alive}
    \If{$\lnot \code{HasSpace}(\DE{return}, e)$}
    \State{\Goto{endPosition}}
    \EndIf
    \State{$\DE{return} := \DE{return} \cup \{e\}$}
    \EndFor
    \State{\Return if oldest message had all live records refreshed\label{endPosition}}
    \EndFunction
\end{algorithmic}
\caption{\label{fig:sendrecordhelpers}Helper Methods to Send Record}
\end{figure}

\newpage
% API
\begin{figure}[!htb]
  \footnotesize
  \begin{algorithmic}[1]
    \Function{StartTransaction}{}
      \State{$\tbuild := \tuple{\seqtlocal, \emptyset, \emptyset}$}
      \State{$\seqtlocal := \seqtlocal + 1$}
    \EndFunction\\

    \Function{CommitTransaction}{}
      \State{$\transaction := \code{GenerateTransaction}(\tbuild)$}
      \State{$\PendingTransact.\code{add}(\transaction)$}
      \State{$\code{DoCommunication}()$}
    \EndFunction\\

    \Function{CreateNewKV}{$k, \id$}
      \If{Key $k$ does not already exist}
        \State{\Return{$\code{SendRecord}(\tuple{k,\id})$}}
      \EndIf
      \State{\Return{Already Has Key $k$}}
    \EndFunction\\
    
    \Function{Update}{}
      \State{$\mathsf{newMsgs} :=$ Get new messages from server using $\getmsg$}
      \If{Had Server Timeout}
        \ForAll{$\id \in$ Known arbitrators}
          \State{$\code{SendLocally}$($null, \id$)}
        \EndFor
        \State{\Return{}}
      \EndIf
      \State{$\code{ValidateandUpdate}(\mathsf{newMsgs})$}
      \State{$\code{DoCommunication}()$}
    \EndFunction\\

    \Function{Put}{$k,v$}
      \State{$\code{CheckHasSameArbitrator}(k, \KV{\tbuild} \cup \MYG{\tbuild})$}
      \State{$\tbuild := \tuple{\stlocaltbuild, \KV{\tbuild} \cup \{\tuple{k,v}\}, \MYG{\tbuild}}$}
    \EndFunction\\

    \Function{GetCommitted}{$k$}
      \State{\Return $\committed[k]$}
    \EndFunction\\

%    \Function{GetSpeculative}{$k$}
%      \State{\Return $\speculated[k]$}
%    \EndFunction\\

    \Function{GetCommittedAtomic}{$k$}
      \State{$\code{CheckHasSameArbitrator}(k, \KV{\tbuild} \cup \MYG{\tbuild})$}
      \State{$\MYG{\tbuild}:=\MYG{\tbuild}\cup \{\tuple{k,\committed[k]}\}$}
      \State{$\tbuild := \tuple{\stlocaltbuild, \KV{\tbuild}, \MYG{\tbuild}}$}
      \State{\Return $\committed[k]$}
    \EndFunction

%    \Function{GetSpeculativeAtomic}{$k$}
%      \State{$\code{CheckHasSameArbitrator}(k, \KV{\tbuild} \cup \G{\tbuild})$}
%      \State{$\G{\tbuild}:=\G{\tbuild}\cup \{\tuple{k,\speculated[k]}\}$}
%      \State{$\tbuild := \tuple{\stlocaltbuild, \KV{\tbuild}, \G{\tbuild}}$}
%      \State{\Return $\speculated[k]$}
%    \EndFunction
  \end{algorithmic}
\caption{\label{fig:clientapi}Client Public API}
\end{figure}

\newpage
% Communication
\begin{figure}[!htb]
  \footnotesize
  \begin{algorithmic}[1]
    \Function{ReceiveLocally}{$\tuple{\transaction, \slastseen}$}
      \If{$\transaction \neq null \land $ Has not seen $\transaction$ before}
        \State{$\NewArb := \code{Arbitrate}(\{\transaction\})$}
        \State{$\PendingArbitration.\code{addAll}(\NewArb)$}
        \State{$\de{} := \NewArb.\code{getFront}()$}
        \If{$\de{}$ is a commit}
          \State{$\tuple{\sserver,\arbLocalId, \tLocalId, \KV{}} := \de{}$}
          \State{Update $\committed$ with $\KV{}$}
        \EndIf
      \EndIf
      \State{$\ArbSet := $ all live $\commit$ and $\abort$ where $\idarblocal= \localid$}
      \State{\Return{$\{\de{}|\de{} \in \ArbSet \land \slastseen < \sarblocal\}$}}
    \EndFunction\\

    \Function{SendLocally}{$\tuple{\sserver, \stlocal, \id, \KV{}, \MYG{}}, \idrec$}
      \State{$\LDat := \tuple{\tuple{\sserver, \stlocal, \id, \KV{}, \MYG{}}$, last $\sarblocal$ seen from $\id$ $}$}
      \State{Send $\LDat$ to $\idrec$ via \code{ReceiveLocally}}
      \State{$\newArbitration :=$ Returned $\{\de{}\}$ from \code{ReceiveLocally}}
      \If{Cannot Communicate Locally with $\id\lor$ Had Failure}
        \State{\Return{$\false$}}
      \EndIf
      \ForAll{$\de{} \in \newArbitration$}
        \State{$\code{processKVStoreRecord}(\de{})$}
      \EndFor
      \State{$\code{processKVStore()}$}
      \State{\Return{$\true$}}
    \EndFunction
  \end{algorithmic}
\caption{\label{fig:localcommunication}Local Communication Helper Functions}
  \end{figure}
  
\begin{figure}[!htb]
  \footnotesize
  \begin{algorithmic}[1]

    \Function{DoCommunication}{}
      \While{$|\PendingTransact| > 0 \lor |\PendingArbitration| > 0$}
        \If{$|\PendingArbitration| > 0$}
          \State{$\de{} := \PendingArbitration.\code{getFront}()$}
        \ElsIf{$|\PendingTransact| > 0$}
          \State{$\de{} := \PendingTransact.\code{getFront}()$}
        \EndIf            
        \State{Update $\sserver$ of $\de{}$ to $\seqnume$ of new message}
        \State{$\didSend:=\code{SendRecord}(\de{})$}

        \If{$\didSend$}
          \State{//Remove from appropriate list}
          \State{$\PendingArbitration.\code{remove}(\de{})$}
          \State{$\PendingTransact.\code{remove}(\de{})$}
        \ElsIf{Had Server Timeout}
          \ForAll{$\de{} \in \PendingTransact$} \label{haderror}
            \If{$\lnot$ $\code{SendLocally}(\de{}, $arbitrator $\id$ of $\de{})$}
              \State{//Stop sending to preserve ordering.}
              \State{Break}
            \Else
              \State{$\PendingTransact.\code{remove}(\de{})$}
            \EndIf
          \EndFor
          \State{Break}  
        \EndIf
      \EndWhile
    \EndFunction
  \end{algorithmic}
\caption{\label{fig:uppercommunication}Key-Value Store Communication Functions}
\end{figure}

\newpage
% Record Handlers
\begin{figure}[!htb]
  \footnotesize
  \begin{algorithmic}[1]

    % \Function{processAbort}{$\tuple{\sserver,\arbLocalId, \tLocalId}$}
    \Function{processAbort}{$\abort$}
      \State{//No Action must be taken here}
    \EndFunction\\

    \Function{processCommit}{$\commit$}
      \If{Client not seen $\commit$ before }
        \State{$\UnprocessedCom:=\UnprocessedCom \cup \{\commit\}$}
      \EndIf
    \EndFunction\\

    \Function{processTransaction}{$\transaction$}
      \If{Client not seen $\transaction$ before and is the arbitrator}
        \State{$\UnprocessedTran:=\UnprocessedTran \cup \{\transaction\}$}
      \EndIf
    \EndFunction\\

    \Function{processNewKey}{$\tuple{\mathsf{k}, \id}$}
      \If{$\id = \localid$}
        \State{Add self to be arbitrator for $k$}
      \EndIf
    \EndFunction\\

    \Function{processKVStoreRecord}{$\de{}$}
      \If{$\de{}$ is a $\abort$}
        \State{$\code{processAbort}(\de{})$}
      \ElsIf{$\de{}$ is a $\commit$}
        % \State{$\code{processCommit}(\de{}, \seqnume)$}
        \State{$\code{processCommit}(\de{})$}
      \ElsIf{$\de{}$ is $\transaction$}
        \State{$\code{processTransaction}(\de{})$}    
      \ElsIf{$\de{}$ is $\newkey$}
        \State{$\code{processNewKey}(\de{})$}   
      \EndIf    
    \EndFunction
  \end{algorithmic}
\caption{\label{fig:messagehandlerUpper}Key-Value Store Record Handlers}
\end{figure}

% Processing
\begin{figure}[!htb]
  \footnotesize
  \begin{algorithmic}[1]

    \Function{Arbitrate}{$Transactions[] T$}   
      \State{$\ArbRecs := []$}
      \State{$\committedTmp := \committed$}
      \ForAll{$\tuple{s_s, s_l, \id, \KV{}, \MYG{}} \in T,$ not arbitrated on $\land \id = \localid$}
        \If{$\forall \tuple{k,v} \in \MYG{}, \committedTmp[k] = v$}
          \State{$\ArbRecs.\code{add}(\code{GenCommit}(s_s, s_l, \id, \KV{}))$}
          \State{Update $\committedTmp$ with $\KV{}$}
        \Else
          \State{$\ArbRecs.\code{add}(\code{GenAbort}(s_s, s_l, \id))$}
        \EndIf
      \EndFor
      \State{\Return{$\ArbRecs$}}
    \EndFunction\\

%    \Function{Speculate}{}   
%      \State{$\speculated := \committed$}
%      \State{$\UnarbTSet:=$ all live transactions in $\localqueue$}
%      \State{$\UnarbTList:= \UnarbTSet$ sorted by $\sserver$}
%      \State{$\UnarbTList.\code{addAll}(\PendingTransact)$}
%      \ForAll{$\tuple{s_s, s_l, \id, \KV{}, \G{}} \in \UnarbTList$}
%        \If{$\forall \tuple{k,v} \in \G{}, \speculated[k] = v$}
%          \State{Update $\speculated$ with $\KV{}$}
%        \EndIf
%      \EndFor
%    \EndFunction\\


    \Function{processKVStore}{}
      \State{$\NewArb := \code{Arbitrate}(\UnprocessedTran$ sorted by $\sserver$)}
      \State{$\PendingArbitration.\code{addAll}(\NewArb)$}
      \State{$\UnprocessedCom := \UnprocessedCom \cup \{\de{} | \de{} \in \NewArb \land \de{} $is a $\commit \}$}
      \State{$\CList := \UnprocessedCom$ sorted by $\arbLocalId$}     
      \ForAll{$\tuple{\sserver,\arbLocalId, \tLocalId,\KV{}}\in \CList$}
         \State{Update $\committed$ with $\KV{}$}
      \EndFor
%      \State{$\code{Speculate}$}
      \State{$\UnprocessedTran := \UnprocessedCom := \emptyset$}
    \EndFunction
  \end{algorithmic}
\caption{\label{fig:upperprocessing}Transaction Processing}
\end{figure}


==> security.tex <==
\mysection{Privacy}\label{sec:security}

\TOOL provides both privacy and security.
The size of network packets or the records accessed can leak information about a computation.
\TOOL is designed to minimize the information leak by smart home devices.   We first discuss the privacy properties of \TOOL.

\begin{defn}[Privacy]
Let\\
{\footnotesize
\begin{equation*}\begin{split}\vec{x} := \tuple{\getmsg(i),\putmsg(\tuple{i, E(D_i)}),..., \getmsg(i+N-1),\\ \putmsg(\tuple{i+N-1, E(D_{i+N-1})})}
\end{split}\end{equation*}}
\end{defn}
denote a sequential data sequence of length $N$ from a single client.
We say that \TOOL is secure if for any two data request sequences
$\vec{x}$ and $\vec{y}$ of the same length, their request sequences
are computationally indistinguishable to the server.

We do not attempt to hide information that may be revealed through timing,
including the interleavings of requests from different clients.  We
thus prove that \TOOL is oblivious for a single client.  The proof can
be easily extended to executions of multiple clients that share an
interleaving schedule.

To prove the security of \TOOL, let $\vec{x}$ be an access sequence of
size $N$.  In the absence of a resize, the server sees the following
sequence of requests:\vspace{-.4em}

{\footnotesize \begin{equation*}\begin{split}\tuple{\getmsg(i),\putmsg(\tuple{i, E(D_i)})...,\getmsg(i+N-1), \\ \putmsg(\tuple{i+N-1, E(D_{i+N-1})})}\end{split}\end{equation*}}\vspace{-.8em}

Any two sequences of requests length $N$ that start at the same
sequence number $i$ will use the same sequence numbers.
While they will contain different encrypted data, the sequence
of encrypted messages sent by the \putmsg request is
computationally indistinguishable by the definition of encryption.
Note that different requests with the same data will produce entirely
different encrypted messages since no two AES blocks contain the
same counter value.

